Vulnerability-Aware Poisoning Mechanism for Online RL with Unknown Dynamics

Poisoning attacks on Reinforcement Learning (RL) systems could take advantage of RL algorithm's vulnerabilities and cause failure of the learning. However, prior works on poisoning RL usually either unrealistically assume the attacker knows the underlying Markov Decision Process (MDP), or directly apply the poisoning methods in supervised learning to RL. In this work, we build a generic poisoning framework for online RL via a comprehensive investigation of heterogeneous poisoning models in RL. Without any prior knowledge of the MDP, we propose a strategic poisoning algorithm called Vulnerability-Aware Adversarial Critic Poison (VA2C-P), which works for most policy-based deep RL agents, closing the gap that no poisoning method exists for policy-based RL agents. VA2C-P uses a novel metric, stability radius in RL, that measures the vulnerability of RL algorithms. Experiments on multiple deep RL agents and multiple environments show that our poisoning algorithm successfully prevents agents from learning a good policy or teaches the agents to converge to a target policy, with a limited attacking budget.

==> 1.6_example.tex <==
%!TEX root = 0_iclr2021_poisonrl_main.tex

\section{A Real-life Poisoning Example}

% \yc{use this example throughout this paper, to illustrate any new concept in a concrete way. e.g. when talking about white box attack, talking about challenges, etc.}
% \yc{Put this example to introduction?}
Figure XXX illustrates how poisoning happens in a real-life scenario. Consider a simple RL-based content recommendation system, where the user and the content being viewed form the current \emph{state}; the recommended next content is the \emph{action} taken by the RL agent; a positive \emph{reward} is provided to the agent if the user clicks the recommended content. The agent keeps learning from the real user environment by exploring and exploiting, with any modern deep RL algorithm such as A2C, PPO, etc. Since content clicking and viewing are on the users' side and the actions are sent by the server, information will be transferred via network, thus possibly eavesdropped and altered by some adversary. Alternatively, an attacker can even pretend to be a normal user and intendedly make some ``misleading'' clicks. Note that the adversary has various ways to attack, e.g., manipulate the user information, alter the recommended content, change the number of clicks, etc. And the goal of the attack also varies, e.g., induce the agent to recommend some specific content, reduce the recommendation quality in general, etc. Note that in order to improve the attack performance, the attacker needs to consider the long-term results --- how much a user likes a content --- instead of only looking at the current clicks.

The aforementioned attack could also appear in many other applications of RL, which prevents RL systems from successfully learning a good policy, and even posts threats to people who rely on the decisions made by RL systems. 
However, most poisoning researches only focus on SL, or directly apply poisoning techniques of SL to RL. It should be noted, and can be seen from the above example, that poisoning RL is difficult and significantly different from poisoning SL, for (1) either the learner or the attacker knows the underlying environment, and the knowledge they have comes from interactions between the learner and the environment, which is policy-dependent; (2) long-term results should be considered, which requires reasonable policy evaluation; and (3) poisoning may happen in various ways and at heterogeneous aims, including states~\citep{behzadan2017vulnerability}, actions~\citep{pinto2017robust}, rewards~\citep{ma2019policy}, and even the underlying environment~\citep{rakhsha2020policy}.


In this paper, we systematically study poisoning RL, with a novel focus on heterogeneous attacking types.
We summarize all these types of poisoning in our formalization in Section XXX.  
 







==> 4_problem_old.tex <==
%!TEX root = 0_icml2020_poisonrl_main.tex

\section{Poisoning Algorithm}
\label{sec:algos}

In this section, we introduce two practical poisoning algorithms respectively for policy-based and value-based learners. 

Assume a monitoring attacker is conducting $\obs_{\boldsymbol{r}}$-poisoning, and the learner is not aware of the existence of the attacker. We choose non-targeting poisoning.

\subsection{Policy-based Learner}

\subsubsection{White-box (Monitoring) Attacker}

\paragraph{Idea 1: }
Suppose the learner uses vanilla policy gradient and the attacker knows its algorithm parameters. Then the attacking strategy in the $k$-th update is 
\yc{off-policy etr (etr def change)}
\begin{align*}
\begin{aligned}[t]
\label{opt:vpg}
&\boldsymbol{\check{r}}_k = & &\argmin{\boldsymbol{r^\prime}} & & \lobj = \etr(\pi_{\theta_{k+1}}, \boldsymbol{r}_k) \\ 
& & &\text{s.t.} & & \theta_{k+1} = \theta_k + \alpha \nabla_{\theta_k} \etr(\pi_{\theta_{k}}, \boldsymbol{r^\prime}) \\ 
& & &  & & \|\boldsymbol{r^\prime}-\boldsymbol{r}_k\| \leq \epsilon
\end{aligned}
\tag{P5}
\end{align*}

Note that for notational simplicity, we use $\etr(\pi_{\theta}, \boldsymbol{r})$ to denote $\hat{\etr}(\pi_{\theta}, \obs(\boldsymbol{r}))$.
Problem~\ref{opt:vpg} is no longer a bi-level optimization problem, since the inner problem is a deterministic update. One can use projected gradient descent to update $\boldsymbol{r}$ by using the chain rule: 
$$
\frac{\partial \lobj}{\partial \boldsymbol{r}^\prime} = \frac{\partial \lobj}{\partial\theta_{k+1}} \frac{\partial{\theta_{k+1}}}{\partial{\boldsymbol{r}^\prime}}.
$$
Note that according to the policy gradient theorem, the gradient of $\etr$ w.r.t. $\theta$ is
$$
\nabla_{\theta} \etr(\pi_{\theta}, \boldsymbol{r}) = \sum_{t=1}^T \nabla_{\theta} \log \pi_{\theta} (a_t|s_t) \sum_{t^\prime=t}^T \gamma^{t^\prime-t} r_t.
$$

\input{algos/w_vpg_alg}

\begin{figure}[h]
	\begin{subfigure}[t]{0.48\columnwidth}
	  \includegraphics[width=\columnwidth]{\fighome/step_attack.png}
	  \caption{stepsize comparison.}
	  \label{fig:stepsize}
	\end{subfigure}
	\hfill
	\begin{subfigure}[t]{0.48\columnwidth}
	  \includegraphics[width=\columnwidth]{\fighome/step_attack_budget.png}
	  \caption{budget comparison.}
	  \label{fig:step_budget}
	\end{subfigure}
	\caption{Algorithm~\ref{alg:wb_poison}}
\end{figure}



\paragraph{Idea 2:}


\begin{align*}
\begin{aligned}[t]
\label{opt:online}
    &\boldsymbol{\check{r}}_k = & &\argmin{\boldsymbol{r^\prime}} & & \lobj = \| \theta_{k+1} - \theta^\dag_{k} \| \\ 
	& & &\text{s.t.} & & \theta_{k+1} = \theta_k + \alpha \nabla_{\theta_k} \etr(\pi_{\theta_{k}}, \boldsymbol{r^\prime}) \\ 
	& & &  & & \theta^\dag_{k} = \theta^\dag_{k-1} - \alpha \nabla_{\theta^\dag_{k-1}} \etr(\pi_{\theta^\dag_{k-1}}, \boldsymbol{r}) \\
	& & &  & & \|\boldsymbol{r^\prime}-\boldsymbol{r}_k\| \leq \epsilon
\end{aligned}
\tag{P6}
\end{align*}

\input{algos/w_teach_alg}


\begin{figure}[h]
	\begin{subfigure}[t]{0.48\columnwidth}
	  \includegraphics[width=\columnwidth]{\fighome/comparison_100.png}
	  \caption{with vs without poisoning.}
	  \label{fig:poison}
	\end{subfigure}
	\hfill
	\begin{subfigure}[t]{0.48\columnwidth}
	  \includegraphics[width=\columnwidth]{\fighome/compare_budget.png}
	  \caption{budget comparison.}
	  \label{fig:budget}
	\end{subfigure}
	\caption{Algorithm~\ref{alg:wb_teach}}
\end{figure}

\subsubsection{Black-box (Tapping) Attacker}
The attacker does not know what algorithm the learner is using, and the exact parameters in the learner's model. 


\paragraph{Idea 1: opposite critic.}

By tapping the learner's observation, an attacker is able to train a value network in an off-policy manner. Note that no matter what algorithm the learner uses, it's goal is to maximize the expected rewards of its policy. As a result, the learner tends to choose the actions with higher expected future rewards (Q-values). If a state-action pair whose true Q value is small happens to return high reward, then the learner will be misled and give the action more priority in the next round. An ideal attack could be reversing all the rewards the learner gains. However, it is too expensive. A cheaper solution is, we can increase the future rewards of bad actions, and decrease the future rewards of good actions, where "bad" and "good" are determined by their Q values.

This attacker is similar with the critic in Actor-Critic methods and we call it \textit{opposite critic}. Contradictory to the critic which tells the actor what action is good, the opposite critic forces the actor to take bad actions as good ones, and good actions as bad ones.

\input{algos/b_critic_alg}

\begin{figure}[h]
	\includegraphics[width=\columnwidth]{\fighome/oc_attack.png}
	\caption{Algorithm~\ref{alg:bb_critic}}
\end{figure}

\paragraph{Idea 2: imitation policy teaching.}
As proposed by \citep{liu2017iterative}, machine teaching is still possible when a ``teacher'' does not have access to the model of the ``student''. By observing the input and the output of the model, the teacher can train a separate model that imitates the student's behaviors.

\input{algos/b_teach_alg}


% \paragraph{Idea 3: utilizing transferability.}











==> 4_problem_old2.tex <==
%!TEX root = 0_neurips2020_poisonrl_main.tex

\section{Poisoning Algorithm for Policy Gradient Learners}
\label{sec:algos}

In this section, we introduce two practical poisoning algorithms respectively for white-box (monitoring) poisoning and black-box (tapping) poisoning.

\paragraph{Settings}
Since in most cases, especially in large environments, knowing the underlying MDP is unrealistic, we focus on the attacks aiming to observation. More specifically, suppose the attacker is conducting $\obs_{\boldsymbol{r}}$-poisoning. We choose non-targeted poisoning, because a target policy is not usually available.
Note that the learner is not aware of the existence of the attacker.

\subsection{White-box (Monitoring) Attacker}

Suppose the learner uses Vanilla Policy Gradient (VPG) and the attacker is monitoring its model. Then the attacking strategy in the $k$-th update is 
% \yc{off-policy etr (etr def change)}

\yc{The original problem coming from P2 =======}
\begin{align*}
\begin{aligned}[t]
&\boldsymbol{\check{r}}_k = & &\argmin{\boldsymbol{\check{r}}} & & \sum_{k^\prime}^k \etr_{\pi_{\theta_{k^\prime}}}(\pi_{\theta_{k+1}}, \boldsymbol{r}_{k^\prime}) \\ 
& & &\text{s.t.} & & \theta_{k+1} = \theta_k + \alpha \nabla_{\theta_k} \etr(\pi_{\theta_{k}}, \boldsymbol{\check{r}}) \\ 
& & &  & & \|\boldsymbol{\check{r}}-\boldsymbol{r}_k\| \leq \epsilon
\end{aligned}
\end{align*}
\yc{However, this requires keeping track of all the previous policies and observations, which is impractical. So I only remains the current observation and policy, as shown in Problem\ref{opt:vpg}========}
\yc{Tightness, difficulty}

\begin{align*}
\begin{aligned}[t]
\label{opt:vpg}
&\boldsymbol{\check{r}}_k = & &\argmin{\boldsymbol{\check{r}}} & & \etr_{\pi_{\theta_k}}(\pi_{\theta_{k+1}}, \boldsymbol{r}_k) \\ 
& & &\text{s.t.} & & \theta_{k+1} = \theta_k + \alpha \nabla_{\theta_k} \etr(\pi_{\theta_{k}}, \boldsymbol{\check{r}}) \\ 
& & &  & & \|\boldsymbol{\check{r}}-\boldsymbol{r}_k\| \leq \epsilon
\end{aligned}
\tag{P3}
\end{align*}
\yc{I used limited-budget style here. Hope we can choose a consistent way in the whole paper.}

Note that for notational simplicity, we use $\etr(\pi_{\theta}, \boldsymbol{r})$ to denote $\hat{\etr}(\pi_{\theta}, \obs(\boldsymbol{r}))$.
Problem~\ref{opt:vpg} is no longer a bi-level optimization problem, since the inner problem is a deterministic update. One can use projected gradient descent to update $\boldsymbol{r}$ by using the chain rule: 
$$
\frac{\partial \lobj}{\partial \boldsymbol{\check{r}}} = \frac{\partial \lobj}{\partial\theta_{k+1}} \frac{\partial{\theta_{k+1}}}{\partial{\boldsymbol{\check{r}}}}.
$$
Note that according to the policy gradient theorem, the gradient of $\etr$ w.r.t. $\theta$ is
$$
\nabla_{\theta} \etr(\pi_{\theta}, \boldsymbol{r}) = \sum_{t=1}^T \nabla_{\theta} \log \pi_{\theta} (a_t|s_t) \sum_{t^\prime=t}^T \gamma^{t^\prime-t} r_t.
$$

\input{algos/w_vpg_alg}

\begin{figure}[!htbp]
	\begin{subfigure}[t]{0.48\columnwidth}
	  \includegraphics[width=\columnwidth]{\fighome/step_attack.png}
	  \caption{stepsize comparison.}
	  \label{fig:stepsize}
	\end{subfigure}
	\hfill
	\begin{subfigure}[t]{0.48\columnwidth}
	  \includegraphics[width=\columnwidth]{\fighome/step_attack_budget.png}
	  \caption{budget comparison.}
	  \label{fig:step_budget}
	\end{subfigure}
	\caption{Algorithm~\ref{alg:wb_poison}}
\end{figure}





\subsection{Black-box (Tapping) Attacker}
The attacker does not know what algorithm the learner is using, and the exact parameters in the learner's model. 


By tapping the learner's observation, an attacker is able to train a value network in an off-policy manner. Note that no matter what algorithm the learner uses, it's goal is to maximize the expected rewards of its policy. As a result, the learner tends to choose the actions with higher expected future rewards (Q-values). If a state-action pair whose true Q value is small happens to return high reward, then the learner will be misled and give the action more priority in the next round. An ideal attack could be reversing all the rewards the learner gains. However, it is too expensive. A cheaper solution is, we can increase the future rewards of bad actions, and decrease the future rewards of good actions, where "bad" and "good" are determined by their Q values.

In other words, according to Equation~\ref{eq:off_policy}, the learner will increase $\pi(a|s)$ if its evaluation of $Q(s,a)$ becomes relatively higher, decrease $\pi(s,a)$ otherwise. Even if the learner may fail to evaluate $Q(s,a)$ correctly, and different learning rates influence the learning results, the attacker is very likely to manipulate the learner's policy by manipulating the rewards.

This poisoning method is similar with the critic in Actor-Critic methods and we call it \textit{opposite critic}. Contradictory to the critic which tells the actor what action is good, the opposite critic forces the actor to take bad actions as good ones, and good actions as bad ones.

To formalize the idea of opposite critic, we first define a set of ``bad choices''.
\begin{definition}[Bad Timesteps]
	For a trajectory $s_1,a_1,r_1,s_2,\cdots,s_t,a_t,r_t,\cdots$, define the \textit{bad timesteps set} $\badset$ as the timesteps $t$ where $a_t$ is a worse-than-average choice, i.e., $$\badset(Q) = \{ t: Q(s_t,a_t) < \frac{1}{|\actions|} \sum_{a\in \actions} Q(s_t,a) \},$$ where $Q$ is the action-value function.
\end{definition}

The main idea of opposite critic is to maximize the future rewards (approximated Q value) of the choices made in bad timesteps, and minimize the future rewards of other (good) choices.


Problem~\ref{opt:op_c} shows the opposite-critic objective for the $k$-th iteration. Note that the inner optimization problem about $\valpara_k$ does not involve $\boldsymbol{\check{r}}$, so it is not a difficult bi-level optimization problem. One can solve $\valpara_k$ first using the existing $\obs_k$, then solve $\boldsymbol{\check{r}}$ using $\valpara_k$.
\begin{align*}
\begin{aligned}[t]
\label{opt:op_c}
&\boldsymbol{\check{r}}_k = & & \argmin{\boldsymbol{r}^\prime} & & \sum_{t\notin W(Q_{\valpara_k})} \sum_{t^\prime=t}^T \gamma^{t^\prime-1} \check{r}_t - \sum_{t\in W(Q_{\valpara_k})} \sum_{t^\prime=t}^T \gamma^{t^\prime-1} \check{r}_t  \\ 
& & &\text{s.t.} & & \valpara_k = \argmin{\valpara} \sum_{(s,a,s^\prime) \in \obs_k} \big(r + \max_{a^\prime}Q_{\valpara_{k-1}}(s^\prime,a^\prime) - Q_{\valpara}(s,a) \big)^2 \\ 
& & &  & & \|\boldsymbol{\check{r}}-\boldsymbol{r}_k\| \leq \epsilon
\end{aligned}
\tag{P4}
\end{align*}


\input{algos/b_critic_alg}

\begin{figure}[h]
	\begin{subfigure}[t]{0.48\columnwidth}
	  \includegraphics[width=\columnwidth]{\fighome/oc_attack.png}
	  \caption{VPG.}
	  \label{fig:stepsize}
	\end{subfigure}
	\hfill
	\begin{subfigure}[t]{0.48\columnwidth}
	  \includegraphics[width=\columnwidth]{\fighome/PPO_bb_cartpole.png}
	  \caption{PPO.}
	  \label{fig:step_budget}
	\end{subfigure}
	\caption{Algorithm~\ref{alg:bb_critic}}
\end{figure}

\yc{robust radius, vulnerability of RL algorithms
https://arxiv.org/pdf/1706.03922.pdf}
% \paragraph{Idea 3: utilizing transferability.}











==> 5_theory.tex <==
%!TEX root = 0_neurips2020_poisonrl_main.tex
\vspace*{-0.5em}
\section{Measuring Vulnerability of RL Algorithms}
\label{sec:vulnerability}
\vspace*{-0.5em}

Definition~\ref{def:stable_radius_update} measures the stability of one update based on policy discrepancy. But it is not obvious whether the rewards change drastically due to the attacks.
% With different distribution distance measures, the interpretation of stability could vary. 
Proposition~\ref{prop:reward_drop} provides a guarantee on the performance of the poisoned policy $\poison{\pi}^\prime$, compared with the un-poisoned new policy $\pi^\prime$. 
\begin{proposition}
\label{prop:reward_drop}
  For an update of stochastic policy $\pi^\prime = \lalg(\pi, \obs)$, if its $\delta$-stability radius is $\varepsilon$ with the total variance measure, then any poisoning effort smaller than $\varepsilon$ on $\victim$ will cause the reward drop by no more than
  \begin{equation}
    \frac{4 \delta^2\gamma |\max_{s,a} A_{\pi^\prime}(s,a)|}{(1-\gamma)^2} + 2\delta \mathbb{E}_{s\sim \pi^\prime} [\max_a  A_{\pi^\prime} (s,a)] - \mathbb{E}_{s,a\sim \pi^\prime} [A_{\pi^\prime} (s,a) ]
  \end{equation}
  where $\gamma$ is the discount factor, and $A$ is the advantage function, i.e., $A_\pi(s,a) = Q_\pi(s,a) - V_\pi(s,a)$.
\end{proposition}
Proposition~\ref{prop:reward_drop} shows that if the attack power is within the stability radius, the reward of the poisoned policy will not be influenced too much.
which also explains the motivation behind our proposed vulnerability-aware attack.
The proof is in Appendix~\ref{app:proof_drop}.

With the one-update stability measure, we are able to formally define the stability radius of an RL algorithm w.r.t. an MDP.
\begin{definition}[Stability Radius w.r.t an MDP]
\label{def:stable_radius_mdp}
The $\delta$-stability radius of an algorithm $\lalg$ in an MDP $\mdp$ is defined as the minimal stability radius of all observations drawn from the MDP, and all possible policies in policy space $\Pi$.
If $\lalg$ is on-policy, then $\stable(\lalg, \mdp) = \min_{\pi\in\Pi, \obs\sim\pi} \stable(\lalg, \pi, \obs) $;
if $\lalg$ is off-policy, then $\stable(\lalg, \mdp) = \min_{\pi\in\Pi, \obs \sim \overline{\pi}} \stable(\lalg, \pi, \obs) $, where $\overline{\pi}$ is the behavior policy;
\end{definition}

We also present a counterpart of stability radius in test time, namely \textit{robustness radius} in Appendix~\ref{app:robust_radius}, as well as a comparison of vulnerability between supervised learning and RL in Appendix~\ref{app:compare}. Stability radius and robustness radius together provide a principled way to measure vulnerability of RL algorithms, respectively in training time and test time.

% (1) In contrast with test time robustness where robust means a perturbation on input will not cause the change of output, an algorithm is stable if a perturbation on training data will not cause the model to be different with the model that it should have gained with clean training data.

% (2) An RL algorithm $\lalg$ dealing with a deterministic policy $\pi$ is stable against perturbation on one trajectory smaller than $\stable(\lalg, \pi, \tau)$.

% (3) For an RL algorithm $\lalg$ with a stochastic policy $\pi$, if its $\delta$-stability radius on a trajectory $\tau$ is $\varepsilon$, then any perturbation within $\varepsilon$ on $\tau$ will cause reward drop by no more than
% \begin{equation}
%   \frac{4\delta^2\gamma \max_{s,a} A_\pi(s,a)}{(1-\gamma)^2}   
%   - \mathbb{E}_{s,a\sim \pi}[A_\pi(s,a)] - 2\delta \mathbb{E}_{s\sim \pi}[\sum_{a} A_\pi(s,a)] 
% \end{equation} 


==> 8_general.tex <==
%!TEX root = 0_iclr2021_poisonrl_main.tex
\vspace*{-0.8em}
\section{Problem Formulation for Poisoning Online RL}
\label{sec:problem-form}
In this section, we formulate the problem of poisoning in online RL through the lens of optimization. 
% We will illustrate its differences and additional challenges compared to poison in supervised learning. 
\yc{A little formulation, targeted and non-targeted, various poisoning types}

We deliberately formulate the optimization problem to be as generic as possible, covering non-targeted and targeted poison objective and all 3 poison target types. 
% We also consider the more challenging scenario of a monitoring attacker, different from the omniscient attacks assumed in most of the previous works.

% \vspace*{-0.8em}
\begin{figure}[htbp]
\vspace*{-0.8em}
    \begin{subfigure}[t]{0.32\columnwidth}
      \includegraphics[width=\columnwidth]{\fighome/examples/obs_attack.pdf}
      \caption{Poison observation $(\obs_{\boldsymbol{r}},\obs_{\boldsymbol{s}})$ }
      \label{sfig:obs}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.32\columnwidth}
      \includegraphics[width=\columnwidth]{\fighome/examples/mdp_attack.pdf}
      \caption{Poison MDP $(\mdp_\rewards, \mdp_\dynamics)$}
      \label{sfig:mdp}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.32\columnwidth}
      \includegraphics[width=\columnwidth]{\fighome/examples/exe_attack.pdf}
      \caption{Poison Executor $\exe_{\boldsymbol{a}}$}
      \label{sfig:exe}
    \end{subfigure}
    \vspace*{-0.5em}
    \caption{{\small{The online poisoning vs learning.
    Blue solid lines denote the learning processes, while red dashed lines denote the poisoning processes.
    % \fh{polish}
    % Green framed $M_k$ and $O_k$ denote the underlying un-poisoned model and observations.
    % Blue framed policies $\pi_k$'s denote learner's models; the learner generates policy $\pi_k$ through (poisoned) observations $O_k$ and previous (poisoned) policy $\pi_{k-1}$.
    % Red framed objects denote the poisoned. 
    In iteration $k$, the learner uses its previous policy $\pi_{k-1}$ to roll out observations $\obs_k$ from current MDP $\mdp_k$, then updates its model and policy by $\pi_k = \lalg(\pi_{k-1}, \obs_k) = {\mathrm{argmax}_{\pi}} \lobj(\pi, \pi_{k-1}, \obs)$. The attacker may (a) poison observations after they are generated, (b) poison MDP before the learner generates observations, or (c) poison the policy when it is used to generate observations. Among these three scenarios, $\obs_k$ is always influenced by the attack, thus denoted as $\poison{\obs}_k$.
    %where green frames stand for the ground-truth, blue frames stand for the learner's models, red frames stand for poisoned items, blue lines stand for the learner's algorithm, red dashed lines stand for the attacker's poisoning.
    }}}
    \label{fig:procedure}
    \vspace*{-1em}
\end{figure}
% We formalize the online learning and poisoning process in Procedure~\ref{proc:flow}. 
% \begin{procedure}
%   \caption{Online Poisoning Flow()}
%   \label{proc:flow}
%   Learner initializes its initial policy $\pi_0$ \;
%   \For{$k=1,\cdots,K$}{
%     \tcr{Attacker may poison the MDP $\mdp_k$ to $\poison{\mdp}_k$} \;
%     Learner rollouts $\obs_k$ in $\mdp_k$ ($\poison{\mdp}_k$) with $\pi_{k-1}$ \;
%     \tcr{Attacker may poison the observation $\obs_k$ to $\poison{\obs}_k$} \;
%     Learner updates its policy to $\pi_{k}$ based on $\obs_k$ ($\poison{\obs}_k$)
%   }  
% \end{procedure}


\textbf{Unified Problem Formulation.} 
We introduce Problem~\eqref{opt:general}, a generic \emph{sequential bilevel optimization} for poisoning attacks. 
As detailed in Section~\ref{sec:framework}, the attacker's loss is the learner's value $\aobj=\etr(\poison{\pi})$ if poisoning is non-targeted, and  $\aobj=\mathrm{distance}(\poison{\pi}, \pi^\dag)$ if poisoning is targeted at $\pi^\dag$.
% Our optimization problem covers the online learning and poisoning procedure under all three poison target types, illustrated in Figure~\ref{fig:procedure}. 
We use $\victim$-poisoning to collectively denote any target types of the poisoning, where $\victim \in \{ \mdp_\rewards, \mdp_\dynamics, \obs_{\boldsymbol{r}}, \obs_{\boldsymbol{s}}, \exe_{\boldsymbol{a}} \}$, illustrating the generality of our formulation.
The online poisoning process is visualized in Figure~\ref{fig:procedure}, which shows $\obs_k$ is poisoned to $\poison{\obs}_k$, conditioned on $\poison{\victim}_k$, regardless of the target type.
Therefore, at iteration $k$, the optimal 
subsequent
 poisoning $\poison{\victim}_{k}, \poison{\victim}_{k+1}, \cdots, \poison{\victim}_K$ are given by the optimal solution of Problem~\eqref{opt:general}.
\begin{align*}
\begin{aligned}[t]
\label{opt:general}
    % &\argmin{\substack{\poison{\victim}_k \in  \mathcal{B}_\epsilon(\victim_k) \\ k=1,\cdots,K}} 
    &\argmin{\poison{\victim}_k, \cdots, \poison{\victim}_K} 
    & & \sum\nolimits_{j=k}^K  \aobj(\poison{\pi}_j)\\
    &s.t. & & \poison{\pi}_{j} = {\mathrm{argmax}_{\pi}} \lobj(\pi, \pi_{j-1}, \poison{\obs}_j | \poison{\victim}_j) , \forall k\leq j \leq K   & \text{\small{(learner's poisoned learning)}}\\
    & & & \sum\nolimits_{j=k}^K \bm{1}\{  \poison{\victim}_j \neq \victim_j \}   \leq \budget  & \text{\small{(limited-budget)}}\\
    &  & & \effort(\victim_j, \poison{\victim}_j) \leq \power, \forall k\leq j \leq K   & \text{\small{(limited-power)}}
\end{aligned}
\tag{Q}
\end{align*}

At each iteration, the learner attempts to obtain a policy that maximizes the objective function $\lobj$ as shown in condition ``(learner's poisoned learning)''.
For example, the objective function for TRPO is $\pi_k = \mathrm{argmax}_{\pi} [ \hat{\mathbb{E}}_t[\frac{\pi(a_t|s_t)}{\pi_{k-1}(a_t|s_t)} \hat{A}_t] - C D^{\max}_{\mathrm{KL}} (\pi_{k-1}, \pi) ]$, where $\hat{A}$ is related with $\obs_k$, and $C, D^{\max}_{\mathrm{KL}}$ are defined in the paper~\citep{schulman2015trust}.


To truthfully represent the real-world scenarios, we consider \emph{attacker's constraints} in two forms: 
(1) the \emph{attack power} $\power$ restricts the maximum change $\effort(\victim_k, \poison{\victim}_k)$ in one iteration, which can be defined by any distance metric (e.g., $\ell_p$-norm),  in condition ``(limited-power)'' and
(2) the \emph{attack budget} $\budget$ restricts the number of iterations that the attacker could attack, in condition ``(limited-budget)''.

 


\textbf{%Problem~\eqref{opt:general} Is 
 Difficulty in Sequential Bilevel Optimization.}  In supervised learning, the poison attacker solves a \emph{bilevel optimization problem} since the attacker, when making the decision of how to poison, has to solve an optimization problem to predict how the learner reacts to the poison injected~\citep{munoz2017towards}. 
Problem~\eqref{opt:general} in online RL is even more challenging as the attacker has to predict how the learner reacts to the poison not only at the current iteration $k$, but also for all future iterations $k+1,\ldots$, since all decisions made at current time will have consequences in the future. 
As a result, Problem~\eqref{opt:general} in online RL is a \emph{sequential bilevel optimization problem}, much more challenging than in the supervised learning setting.


% \textbf{Example Problem Attacking Policy Gradient Learners}
% To illustrate the generic optimization of Problem~\eqref{opt:general} in an instantiated RL problem, we describe \eqref{opt:general} under a prevalent RL agent, policy gradient learner. 
% \fh{Put the optimization here, without relaxation. Now the learner doesn't solve an argmax, it just uses its algorithm.}


% \begin{align*}
% \begin{aligned}[t]
% \label{opt:pgl}
%     % &\argmin{\substack{\poison{\victim}_k \in  \mathcal{B}_\epsilon(\victim_k) \\ k=1,\cdots,K}} 
%     &\argmin{\poison{\victim}_1, \poison{\victim}_2, \cdots, \poison{\victim}_K} 
%     & & \sum\nolimits_{k=1}^K  ??  \\
%     &s.t. & & \poison{\pi}_{k} = ?? , \forall k   & \text{\small{(learner's poisoned learning)}}\\
%     & & & \sum\nolimits_{k=1}^K \bm{1}\{  \poison{\victim}_k \neq \victim_k \}   \leq \budget, \forall k  & \text{\small{(limited-budget)}}\\
%     &  & & \effort(\victim_k, \poison{\victim}_k) \leq \power, \forall k & \text{\small{(limited-power)}}
% \end{aligned}
% \tag{I}
% \end{align*}

%The first constraint in Problem~\eqref{opt:general} denotes the learner's objective, however the generated policy by the learner's algorithm $\lalg(\pi_{k-1}, \poison{\obs}_k | \poison{\victim}_k)$ does not necessarily achieve the maximization of the objective function.

% \yc{milder, what are the options, conditions for the problem to be tractable, argue that the conditions are not realistic}
% Directly solving the \emph{sequential bilevel optimization problem}~\eqref{opt:general} is challenging, since it requires knowledge of the true MDP asend the observations in all iterations \fh{?}. \fh{Delete this paragraph.}


% Directly solving the \emph{sequential bilevel optimization problem}~\eqref{opt:general} is challenging.
\textbf{Possible Directions in Addressing Problem~\eqref{opt:general}}

\emph{Case (1)} Under the often unrealistic setting of attacker being omniscient, the attacker can exactly compute all observations $\poison{\obs}_{k:K}$ based on environment dynamics. 
% and the environment is deterministic (or the environment is stochastic, but the random seed is known by the attacker), 
Then, Problem~\eqref{opt:general} reduces to a fully-online case of the supervised learning attack studied by \citet{wang2018data} where the training data stream is known to the attacker. 
% In this scenario, the attacker can find the optimal solution of \eqref{opt:general} before the learner starts learning. %, which is called ``\textit{offline poisoning}''. 
Note that even in this case, solving Problem~\eqref{opt:general} is NP-hard if $C \ll K$. 
% However, the omniscient attacker assumption is unrealistic especially for large and complex environments. 

\vspace*{-0.5em}
\emph{Case (2)} For a non-omniscient attacker, future observations are not available. But it might be possible for the attacker to train a prediction model~\citep{junhyuk2015action} of the environment in advance, and use the estimated model to predict future observations of the learner based on its current policy. However, the computational cost could be very high.
% Problem~\eqref{opt:general} can not be directly solved, because $\poison{\victim}_k$ should be determined before observing $\{\poison{\obs}_{k^\prime}\}_{k^\prime=k+1}^K$. 

\vspace*{-0.5em}
\emph{Case (3)} If the non-omniscient attacker can not study the environment ahead of time, and can only learn along with the learner, then predicting the future becomes prohibitive.
In this case, the attacker has to sequentially make two decisions: ``\textbf{when to attack}'', and ``\textbf{how to attack}'', in order to approximately solve Problem~\eqref{opt:general}.
% , which is called ``\textit{online poisoning}'' \fh{why do we have 'which is called online poisoning'?}. 

% We aim to tackle the more challenging online poisoning problem \fh{which online poisoning problem? Its reference not clear.} 
We aim to tackle the more challenging but practical \emph{Case (3)} and propose a poisoning algorithm described in Section~\ref{sec:problem}, with a focus on policy-gradient learners for demonstration purpose.
% Therefore, in practice, Problem~\ref{opt:general} should be relaxed to be tractable. 

% \paragraph{Problem Relaxation}
% Since $\{\poison{\obs}_{k^\prime}\}_{k^\prime=k}^K$ are not available when computing $\poison{\victim}$, we relax Problem~\ref{opt:general} to Problem~\ref{opt:relax}, where the current poisoning does not rely on the future observation.
% \begin{align*}
% \begin{aligned}[t]
% \label{opt:relax}
%     &\argmin{\poison{\victim}_k} & & \sum_{k^\prime=1}^k  \aobj(\hat{\pi}_{k^\prime}, \victim_{k^\prime}) + \lambda \effort(\victim_k, \poison{\victim}_k)   \\
%     &s.t. & & \hat{\pi}_k = \argmax{\pi} \Hquad \lobj(\pi, \poison{\victim}_k)
% \end{aligned}
% \tag{P2}
% \end{align*}

% However, Problem~\ref{opt:relax} is still challenging, as a bi-level optimization problem, even if the learner's model is known to the attacker. We propose some practical algorithms in Section~\ref{sec:algos} that can efficiently solve the poisoning problem.



% \paragraph{Targeted poisoning.}
% The attacker wants to force the learner to learn a targeted policy $\pi^\dag$ that is given.  
% Then the poisoning is done by solving the following optimization problem

% \begin{align*}
% \label{opt:target}
%     &\poison{\victim}_k = & &\argmin{\victim^\prime} & &\effort(\victim_k, \victim^\prime)    \\
%     & & &s.t. & & \mathrm{dist} (\hat{\pi}_k, \pi^{\dag}) \leq \epsilon  \\
%     & &  & & & \hat{\pi}_k = \argmax{\pi} \Hquad \lobj(\pi, \victim^\prime) 
% \tag{P1}
% \end{align*}
% where $\mathrm{dist}(\cdot, \cdot)$ is a function measuring the distance between two policies (one can use $p$-norm, KL-divergence, and etc.).
% \yc{not necessary to know the model parameters}

% \paragraph{Non-targeted poisoning.} 
% The attacker aims to let the learner get as less reward as possible. 

% \begin{align*}
% \label{opt:ntarget}
%     &\poison{\victim}_k = & &\argmin{\victim^\prime} & &   \lobj(\hat{\pi}_k, \victim)   \\
%     & & &s.t. & & \effort(\victim_k, \victim^\prime) \leq \epsilon  \\
%     & &  & & & \hat{\pi}_k = \argmax{\pi} \Hquad \lobj(\pi, \victim^\prime) 
% \tag{P2}
% \end{align*}

% \paragraph{A general formalization.} 
% Both the targeted problem and non-targeted problem can be converted and formalized into the following problem
% \begin{align*}
% \label{opt:general}
%     &\poison{\victim} = & &\argmin{\victim^\prime} & &  \aobj(\hat{\pi}, \victim) + \lambda \effort(\victim, \victim^\prime)   \\
%     & & &s.t. & & \hat{\pi} = \argmax{\pi} \Hquad \lobj(\pi, \victim^\prime)  
% \tag{P3}
% \end{align*}
% where $\aobj(\hat{\pi}, \victim) = \mathrm{dist} (\hat{\pi}, \pi_{\dag})$ for targeted poisoning, and $\aobj(\hat{\pi}, \victim) = \lobj(\hat{\pi}, \victim)$ for non-targeted poisoning, denoted by $\aobjt$ and $\aobjnt$ respectively. Note that there exists a $\lambda$ that makes (\ref{opt:general}) equivalent to (\ref{opt:target}) or (\ref{opt:ntarget}).
% \fh{drew the figure with the colored arrows. this paragraph was in the previous section as well.}
% \begin{align*}
% \begin{aligned}[t]
% \label{opt:general}
%     &\argmin{\poison{\victim}_1, \cdots, \poison{\victim}_K} & & \sum_{k=1}^K  \aobj(\hat{\pi}_k, \victim_k) + \lambda \effort(\victim_k, \poison{\victim}_k)   \\
%     &s.t. & & \hat{\pi}_k = \argmax{\pi} \Hquad \lobj(\pi, \poison{\victim}_k), k=1,\cdots,K
% \end{aligned}
% \tag{P1}
% \end{align*}
% \vspace*{-0.5em}

% Note that the lower level optimization problem is not necessarily an argmax function, and in this case the learners poisoned learning is $\poison{\pi}_{k} = \lalg(\pi_{k-1}, \poison{\obs}_k | \poison{\victim}_k)$.
% change to the following?
% \yc{The lower level problem expression is not accurate. I don't think this problem can be viewed as a general bi-level optimization problem}
% where $\mathcal{B}_\epsilon(\victim_k) = \{ \victim |  \effort(\victim_k, \victim) \leq \epsilon \}$.
% Note that $\lalg(\pi_{k-1}, \poison{\victim}_k) = \lalg(\pi_{k-1}, \poison{\obs}_k)$ if the attacker poisons the observation or executor, $\lalg(\pi_{k-1}, \poison{\victim}_k) = \lobj(\pi, \obs_k | \obs_k \sim\poison{\mdp}_k)$ if the attacker poisons the environment. 




==> algos/b_critic_alg.tex <==
%!TEX root = ../0_neurips2020_poisonrl_main.tex

\begin{algorithm}[!ht]
\DontPrintSemicolon
\caption{Opposite Critic}
\label{alg:bb_critic}
  \Input{Poisoning budget $\epsilon$; maximum iteration $maxiter$; two learning rates $\beta_\valpara$ and $\beta_r$}
  \Output{$\poison{\obs}$ with poisoned reward $\poison{\boldsymbol{r}}$}
  Initialize the value network parameters $\valpara_0$ \;
  \For{$k=1,\cdots$}{
    Obtain the recent observation $\obs_k$ \;
    $\valpara_k \gets copy(\valpara_{k-1})$ \;
    \For{$s,a,r,s^\prime \in \obs_k$}{
      $\valpara_k \gets \valpara_k + \beta_\valpara \big(r + \max_{a^\prime}Q_{\valpara_{k-1}}(s^\prime,a^\prime) - Q_{\valpara_k}(s,a) \big) \frac{\partial Q_{\valpara_k}(s,a)}{\partial \valpara_k}$
    }
    Initialize $\poison{\boldsymbol{r}}$ as the original $\boldsymbol{r}$ in $\obs_k$ \;
    \For{$i = 1, \cdots, maxiter$}{
      $\poison{\boldsymbol{r}} \gets \Pi_{\mathcal{B}_\epsilon(\boldsymbol{r})} \Big( \argmin{\boldsymbol{r}^\prime} \sum_{t\notin W(Q_{\valpara_k})} \sum_{t^\prime=t}^T \gamma^{t^\prime-1} \check{r}_t - \sum_{t\in W(Q_{\valpara_k})} \sum_{t^\prime=t}^T \gamma^{t^\prime-1} \check{r}_t \Big)$ \;
      % $\poison{\boldsymbol{r}} \gets \Pi_{\mathcal{B}_\epsilon(\boldsymbol{r})} \big( \argmax{\boldsymbol{r}^\prime} G^-(\boldsymbol{r}^\prime) - G^+(\boldsymbol{r}^\prime) \big)$\;
      % where $G^-(\boldsymbol{r}^\prime) = \underset{\substack{t:a_t=\\ \mathrm{argmin}Q_{\valpara_k}}}{\sum} \sum\limits_{t^\prime=t}^T \gamma^{t^\prime-1} r^\prime_t$\;
      % and $G^+(\boldsymbol{r}^\prime) = \underset{\substack{t:a_t\neq\\ \mathrm{argmin}Q_{\valpara_k}}}{\sum} \sum\limits_{t^\prime=t}^T \gamma^{t^\prime-1} r^\prime_t$\;
      \If{$\poison{\boldsymbol{r}}$ converges}{
        Break \;
      }
    }
    \KwRet{$\poison{\boldsymbol{r}}$} \;
  }
\end{algorithm}

==> algos/b_teach_alg.tex <==
%!TEX root = ../0_icml2020_poisonrl_main.tex

\begin{algorithm}[!ht]
\DontPrintSemicolon
\caption{Imitation Policy Teaching}
\label{alg:bb_teach}
  \Input{Poisoning budget $\epsilon$; maximum iteration $maxiter$; two learning rates $\beta_1$ and $\beta_2$}
  Initialize $\varphi_0$ and $\theta^\dag_0$ randomly \;
  \For{$k=1, \cdots$}{
    Obtain the recent observation $\obs_k$ \;
    Update the target model $\theta^\dag_{k} = \theta^\dag_{k-1} - \alpha \nabla_{\theta^\dag_{k-1}} \etr(\pi_{\theta^\dag_{k-1}}, \boldsymbol{r})$ \;
    \For{$s,a \in \obs_k$}{
      $\varphi_k \gets \varphi_{k-1} - \beta_1 (\pi_{\varphi_{k-1}(s)} - a) \frac{\partial \pi_{\varphi_{k-1}(s)}}{\partial \varphi_{k-1}}$
    }
    Initialize $\poison{\boldsymbol{r}}$ as the original $\boldsymbol{r}$ in $\obs_k$ \;
    $\varphi^\prime \gets copy(\varphi_k)$ \;
    \For{$i = 1, \cdots, maxiter$}{
      $\poison{\boldsymbol{r}}_k \gets \Pi_{\mathcal{B}_\epsilon(\boldsymbol{r})} \Big( \argmin{\boldsymbol{r}^\prime} \Hquad \alpha^2 \nabla_{\varphi^\prime} \etr(\pi_{\varphi^\prime}, \boldsymbol{r}^\prime)^2$ \;
      $ \quad \quad + 2 \alpha \langle \varphi^\prime-\theta^\dag_{k}, \nabla_{\varphi^\prime} \etr(\pi_{\varphi^\prime}, \boldsymbol{r}^\prime) \rangle \Big)$ \;
      $\varphi^\prime \gets \theta_k + \alpha \nabla_{\varphi_k} \etr(\pi_{\varphi_{k}}, \poison{\boldsymbol{r}})$ \;
    }
    Replace $\boldsymbol{r}$ in $\obs_k$ by $\poison{\boldsymbol{r}}$ and return it to the learner 
  }
\end{algorithm}

==> algos/w_teach_alg.tex <==
%!TEX root = ../0_icml2020_poisonrl_main.tex

\begin{algorithm}[!ht]
\DontPrintSemicolon
\caption{Policy Teaching}
\label{alg:wb_teach}
  \Input{Poisoning budget $\epsilon$; maximum iteration $maxiter$; attacker's learning rate $\beta$; learner's initial model $\theta_0$}
  Initialize $\theta^\dag_0 \gets \theta_0$ \;
  \For{$k=1, \cdots$}{
    Obtain the recent observation $\obs_k$ \;
    Obtain the current learner's model $\theta_k$ \;
    Update the target model $\theta^\dag_{k} = \theta^\dag_{k-1} - \alpha \nabla_{\theta^\dag_{k-1}} \etr(\pi_{\theta^\dag_{k-1}}, \boldsymbol{r})$ \;
    Initialize $\poison{\boldsymbol{r}}$ as the original $\boldsymbol{r}$ in $\obs_k$ \;
    $\theta^\prime \gets copy(\theta_k)$ \;
    \For{$i = 1, \cdots, maxiter$}{
      $\poison{\boldsymbol{r}}_k \gets \Pi_{\mathcal{B}_\epsilon(\boldsymbol{r})} \Big( \argmin{\boldsymbol{r}^\prime} \Hquad \alpha^2 \nabla_{\theta^\prime} \etr(\pi_{\theta^\prime}, \boldsymbol{r}^\prime)^2$ \;
      $ \quad \quad + 2 \alpha \langle \theta^\prime-\theta^\dag_{k}, \nabla_{\theta^\prime} \etr(\pi_{\theta^\prime}, \boldsymbol{r}^\prime) \rangle \Big)$ \;
      $\theta^\prime \gets \theta_k + \alpha \nabla_{\theta_k} \etr(\pi_{\theta_{k}}, \poison{\boldsymbol{r}})$ \;
    }
    Replace $\boldsymbol{r}$ in $\obs_k$ by $\poison{\boldsymbol{r}}$ and return it to the learner 
  }
\end{algorithm}

==> fig_disc.tex <==
%!TEX root = 0_neurips2020_poisonrl_main.tex
\vspace*{-0.5em}
\begin{figure}[!htbp]
\centering
	\begin{subfigure}[t]{0.24\columnwidth}
		\centering
		\input{\fighome/disc_plots/cart_vpg.tex}
	% \caption{VPG on CartPole}
	% \label{sfig:vpg_cart}
	\end{subfigure}
	\hfill
	\begin{subfigure}[t]{0.24\columnwidth}
		\centering
		\input{\fighome/disc_plots/walker_vpg.tex}
	% \caption{VPG on CartPole}
	% \label{sfig:vpg_cart}
	\end{subfigure}
	\hfill
	\begin{subfigure}[t]{0.24\columnwidth}
		\centering
		\input{\fighome/disc_plots/cart_ppo.tex}
	% \caption{VPG on CartPole}
	% \label{sfig:vpg_cart}
	\end{subfigure}
	\hfill
	\begin{subfigure}[t]{0.24\columnwidth}
		\centering
		\input{\fighome/disc_plots/walker_ppo.tex}
	% \caption{VPG on CartPole}
	% \label{sfig:vpg_cart}
	\end{subfigure}
\vspace{-1.5em}
\caption{\small{Comparison of policy discrepancies at every iteration. }}
\label{fig:disc}
\end{figure}
\vspace*{-0.5em}

==> fig_poison.tex <==
%!TEX root = 0_neurips2020_poisonrl_main.tex
\vspace*{-0.5em}
\begin{figure}[!htbp]
\centering
	\begin{subfigure}[t]{0.24\columnwidth}
		\centering
		\input{\fighome/vpg_ppo/CartPole_vpg_e=8.0.tex}
	% \caption{VPG on CartPole}
	% \label{sfig:vpg_cart}
	\end{subfigure}
	\hfill
	\begin{subfigure}[t]{0.24\columnwidth}
		\centering
		\input{\fighome/vpg_ppo/Walker2d_vpg_e=2.0_smooth.tex}
	% \caption{VPG on CartPole}
	% \label{sfig:vpg_cart}
	\end{subfigure}
	\hfill
	\begin{subfigure}[t]{0.24\columnwidth}
		\centering
		\input{\fighome/vpg_ppo/Hopper_ppo_e=4.0_smooth.tex}
	% \caption{VPG on CartPole}
	% \label{sfig:vpg_cart}
	\end{subfigure}
	\hfill
	\begin{subfigure}[t]{0.24\columnwidth}
		\centering
		\input{\fighome/vpg_ppo/Walker_ppo_e=4.0_smooth.tex}
	% \caption{VPG on CartPole}
	% \label{sfig:vpg_cart}
	\end{subfigure}

	\vspace*{-1em}
	\begin{subfigure}[t]{0.24\columnwidth}
		\centering
		\input{\fighome/a2c_acktr/CartPole-v0_a2c_e=2.0.tex}
	% \caption{VPG on CartPole}
	% \label{sfig:vpg_cart}
	\end{subfigure}
	\hfill
	\begin{subfigure}[t]{0.24\columnwidth}
		\centering
		\input{\fighome/a2c_acktr/HalfCheetah_a2c_e=1.0.tex}
	% \caption{VPG on CartPole}
	% \label{sfig:vpg_cart}
	\end{subfigure}
	\hfill
	\begin{subfigure}[t]{0.24\columnwidth}
		\centering
		\input{\fighome/a2c_acktr/Hopper_acktr_e=1.0.tex}
	% \caption{VPG on CartPole}
	% \label{sfig:vpg_cart}
	\end{subfigure}
	\hfill
	\begin{subfigure}[t]{0.24\columnwidth}
		\centering
		\input{\fighome/a2c_acktr/Walker_acktr_e=2.0.tex}
	% \caption{VPG on CartPole}
	% \label{sfig:vpg_cart}
	\end{subfigure}
	\vspace*{-1em}
	\caption{\small{Comparison of mean rewards of VPG, PPO, A2C, ACKTR on various environments, with no poisoning, random poisoning, \ourmodtwo and \ourmod. }}
	\label{fig:poison}
\end{figure}
\vspace*{-0.5em}

==> fig_sac.tex <==
%!TEX root = 0_iclr2021_poisonrl_main.tex
\vspace*{-0.5em}
\begin{figure}[!htbp]
\centering
	\begin{subfigure}[t]{0.25\columnwidth}
		\centering
		\input{\fighome/non_target_bb/LunarLander-v2_a2c_action_e=0.1_bb.tex}
	% \caption{VPG on CartPole}
	% \label{sfig:vpg_cart}
	\end{subfigure}
	\hfill
	\begin{subfigure}[t]{0.24\columnwidth}
		\centering
		\input{\fighome/non_target_hybrid/hybrid_CartPole-v0_vpg.tex}
	% \caption{VPG on CartPole}
	% \label{sfig:vpg_cart}
	\end{subfigure}
	\hfill
	\begin{subfigure}[t]{0.24\columnwidth}
		\centering
		\input{\fighome/target/targ_CartPole-v0_a2c.tex}
	% \caption{VPG on CartPole}
	% \label{sfig:vpg_cart}
	\end{subfigure}
	\hfill
	\begin{subfigure}[t]{0.24\columnwidth}
		\centering
		\input{\fighome/target/targ_LunarLander-v2_a2c.tex}
	% \caption{VPG on CartPole}
	% \label{sfig:vpg_cart}
	\end{subfigure}
	\vspace*{-2em}
	\caption{\small{(a) \ourmod also works under black-box setting; (b) hybrid-aim poisoning could be better than single-aim poisoning; (c)(d) \ourmod successfully forces the agent to choose the target policy. }}
	\label{fig:extend}
\end{figure}
\vspace*{-0.5em}

==> figures/compare/compare_CartPole_a2c.tex <==
% This file was created by matplotlib2tikz v0.7.4.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.776470588235294,0.443137254901961,0.443137254901961}
\definecolor{color1}{rgb}{0.662745098039216,0.756862745098039,0.835294117647059}

\begin{axis}[
legend cell align={left},
legend style={at={(0.91,0.5)}, anchor=east, draw=white!80.0!black},
tick align=outside,
tick pos=left,
title={CartPole,A2C,obs 0.3},
x grid style={white!69.01960784313725!black},
xlabel={Iterations},
xmin=-4.9, xmax=102.9,
xtick style={color=black},
y grid style={white!69.01960784313725!black},
ylabel={Progress (\%)},
ymin=3.75091989361905, ymax=104.615545328794,
ytick style={color=black}
]
\path [draw=color0, fill=color0, opacity=0.25]
(axis cs:0,83.4399807407494)
--(axis cs:0,68.7553425332642)
--(axis cs:1,67.5121597497)
--(axis cs:2,65.3445003818112)
--(axis cs:3,61.4404366689898)
--(axis cs:4,57.1570681227505)
--(axis cs:5,50.8712825861069)
--(axis cs:6,45.5729117269267)
--(axis cs:7,37.799103121632)
--(axis cs:8,32.2017894737999)
--(axis cs:9,28.3782779036109)
--(axis cs:10,25.0528561093997)
--(axis cs:11,20.7728381544681)
--(axis cs:12,17.4159744958388)
--(axis cs:13,14.7538112440843)
--(axis cs:14,13.4861378263488)
--(axis cs:15,12.4888026960234)
--(axis cs:16,11.2382972362782)
--(axis cs:17,10.2885160614327)
--(axis cs:18,9.77292896270211)
--(axis cs:19,9.53562880548913)
--(axis cs:20,9.32442109237556)
--(axis cs:21,9.1900560496456)
--(axis cs:22,9.24968998678024)
--(axis cs:23,9.28423667679379)
--(axis cs:24,9.34870308992141)
--(axis cs:25,9.39101664181289)
--(axis cs:26,9.17412463171738)
--(axis cs:27,8.89342971966132)
--(axis cs:28,8.92498029823648)
--(axis cs:29,9.11944081306988)
--(axis cs:30,9.12641734083995)
--(axis cs:31,9.06277942261582)
--(axis cs:32,9.00030384245529)
--(axis cs:33,8.9018023259816)
--(axis cs:34,8.95355462030457)
--(axis cs:35,9.02138463874407)
--(axis cs:36,8.89201664049369)
--(axis cs:37,8.96996997523329)
--(axis cs:38,8.97848156242481)
--(axis cs:39,8.90086031743257)
--(axis cs:40,8.84043311338565)
--(axis cs:41,8.8312997226599)
--(axis cs:42,8.88330960870012)
--(axis cs:43,9.01288146957194)
--(axis cs:44,8.99355748656268)
--(axis cs:45,9.13121515656051)
--(axis cs:46,9.07934443968897)
--(axis cs:47,9.00898830375198)
--(axis cs:48,9.10477888985967)
--(axis cs:49,9.18419195231917)
--(axis cs:50,9.11223213124601)
--(axis cs:51,9.1268110230702)
--(axis cs:52,9.18486459189671)
--(axis cs:53,9.35613216059958)
--(axis cs:54,9.52379480599784)
--(axis cs:55,9.42328670212124)
--(axis cs:56,9.35085964141167)
--(axis cs:57,9.24834024726955)
--(axis cs:58,9.15514752004247)
--(axis cs:59,9.20902943538687)
--(axis cs:60,9.21752462021352)
--(axis cs:61,9.18996984332401)
--(axis cs:62,9.26638372654021)
--(axis cs:63,9.19989912845942)
--(axis cs:64,9.12642025424676)
--(axis cs:65,9.04937565434721)
--(axis cs:66,8.97964646012485)
--(axis cs:67,8.89435139161779)
--(axis cs:68,8.57866332882386)
--(axis cs:69,8.49663856970446)
--(axis cs:70,8.50234166535791)
--(axis cs:71,8.5539834147537)
--(axis cs:72,8.35454123418239)
--(axis cs:73,8.7749885542892)
--(axis cs:74,8.99238528144643)
--(axis cs:75,8.99573967915763)
--(axis cs:76,9.0035517454469)
--(axis cs:77,9.07479697435151)
--(axis cs:78,9.12907536708965)
--(axis cs:79,9.07920970761706)
--(axis cs:80,9.24268987937189)
--(axis cs:81,9.35170585028794)
--(axis cs:82,9.31065881491968)
--(axis cs:83,9.24069214008317)
--(axis cs:84,9.31336179001575)
--(axis cs:85,9.37001807333888)
--(axis cs:86,9.1465227633378)
--(axis cs:87,8.95080044162663)
--(axis cs:88,8.92005644623125)
--(axis cs:89,9.09555363073296)
--(axis cs:90,8.92451995201391)
--(axis cs:91,8.90121834322992)
--(axis cs:92,8.63448198996164)
--(axis cs:93,8.3356755952179)
--(axis cs:94,8.52895885708941)
--(axis cs:95,8.80985466261784)
--(axis cs:96,9.33778470923907)
--(axis cs:97,9.73056289534681)
--(axis cs:98,9.51755012030133)
--(axis cs:98,12.0097777791864)
--(axis cs:98,12.0097777791864)
--(axis cs:97,12.2293368434973)
--(axis cs:96,12.4016173345807)
--(axis cs:95,12.4523650639238)
--(axis cs:94,13.007898714881)
--(axis cs:93,13.7419747965807)
--(axis cs:92,12.9004810423979)
--(axis cs:91,11.9381260766795)
--(axis cs:90,12.1971162357541)
--(axis cs:89,12.03264090925)
--(axis cs:88,12.2609664292679)
--(axis cs:87,12.0497877617886)
--(axis cs:86,11.7623824482468)
--(axis cs:85,11.3035645152901)
--(axis cs:84,11.0231422656332)
--(axis cs:83,10.9446208191182)
--(axis cs:82,11.0539967973758)
--(axis cs:81,10.9084156261209)
--(axis cs:80,10.9648221981687)
--(axis cs:79,10.7049864855772)
--(axis cs:78,10.9329724616767)
--(axis cs:77,11.2256950918452)
--(axis cs:76,11.6631211527656)
--(axis cs:75,11.7896001396949)
--(axis cs:74,12.4018880636354)
--(axis cs:73,13.1192512445156)
--(axis cs:72,13.4708642893023)
--(axis cs:71,12.2651869497643)
--(axis cs:70,11.8088257429342)
--(axis cs:69,11.9144387062876)
--(axis cs:68,11.8730874371023)
--(axis cs:67,11.8126423423519)
--(axis cs:66,11.0374016401102)
--(axis cs:65,10.7305646394604)
--(axis cs:64,10.4239729444537)
--(axis cs:63,10.3244487643195)
--(axis cs:62,10.398160235951)
--(axis cs:61,10.4267404545092)
--(axis cs:60,10.476734359679)
--(axis cs:59,10.5656586802054)
--(axis cs:58,10.5349805867815)
--(axis cs:57,10.8069984150489)
--(axis cs:56,10.6997863032432)
--(axis cs:55,10.7132619468402)
--(axis cs:54,10.7938846541702)
--(axis cs:53,10.5297200266699)
--(axis cs:52,10.3987696534385)
--(axis cs:51,10.4908941047029)
--(axis cs:50,10.4631929510191)
--(axis cs:49,10.3252615530145)
--(axis cs:48,10.4077487631671)
--(axis cs:47,10.3205803265436)
--(axis cs:46,10.3275376554045)
--(axis cs:45,10.408810463137)
--(axis cs:44,10.4285233176144)
--(axis cs:43,10.3101403344149)
--(axis cs:42,10.2608292655843)
--(axis cs:41,10.3094191804072)
--(axis cs:40,10.2607914006171)
--(axis cs:39,10.2399679846425)
--(axis cs:38,10.4901427703618)
--(axis cs:37,10.5851460165713)
--(axis cs:36,10.7156589899575)
--(axis cs:35,10.8184818925183)
--(axis cs:34,10.7887841772052)
--(axis cs:33,10.4187253932849)
--(axis cs:32,10.4447950015248)
--(axis cs:31,10.3627730549995)
--(axis cs:30,10.3764410553904)
--(axis cs:29,10.5907280272387)
--(axis cs:28,10.8526120450532)
--(axis cs:27,11.2799836725726)
--(axis cs:26,11.2882811737465)
--(axis cs:25,11.3005524301227)
--(axis cs:24,11.6606947909746)
--(axis cs:23,12.2985520927943)
--(axis cs:22,13.2765310131801)
--(axis cs:21,14.4946309188785)
--(axis cs:20,15.8229763860294)
--(axis cs:19,17.2838207644308)
--(axis cs:18,18.5588073768674)
--(axis cs:17,20.5634231179434)
--(axis cs:16,22.2826447804861)
--(axis cs:15,23.9817645487359)
--(axis cs:14,26.9508680191462)
--(axis cs:13,30.6289052008057)
--(axis cs:12,34.9403750777209)
--(axis cs:11,39.7682562778124)
--(axis cs:10,44.5789869719166)
--(axis cs:9,52.9162484568317)
--(axis cs:8,59.736267107784)
--(axis cs:7,66.8043359317406)
--(axis cs:6,72.4865316985089)
--(axis cs:5,77.5672440635096)
--(axis cs:4,79.5675653927849)
--(axis cs:3,85.253303017696)
--(axis cs:2,86.2117612276166)
--(axis cs:1,85.6841995136502)
--(axis cs:0,83.4399807407494)
--cycle;

\path [draw=color1, fill=color1, opacity=0.25]
(axis cs:0,51.8753730927767)
--(axis cs:0,48.5246269072234)
--(axis cs:1,49.4647107862529)
--(axis cs:2,51.5656348828178)
--(axis cs:3,54.356071153601)
--(axis cs:4,57.6372137931782)
--(axis cs:5,61.704504336247)
--(axis cs:6,65.62274497501)
--(axis cs:7,69.3429934832771)
--(axis cs:8,74.3805914785306)
--(axis cs:9,77.7742223097503)
--(axis cs:10,80.7635961603475)
--(axis cs:11,83.8657702327849)
--(axis cs:12,86.3609608092412)
--(axis cs:13,88.2649441412615)
--(axis cs:14,89.7562897655948)
--(axis cs:15,91.4277561081106)
--(axis cs:16,92.7387281674098)
--(axis cs:17,93.6899873244943)
--(axis cs:18,94.7778796102284)
--(axis cs:19,95.4126298752077)
--(axis cs:20,96.0581597140529)
--(axis cs:21,96.6293513367282)
--(axis cs:22,96.9347965900243)
--(axis cs:23,97.2413846080631)
--(axis cs:24,97.6911096126988)
--(axis cs:25,98.1206551859049)
--(axis cs:26,98.2099474645068)
--(axis cs:27,98.5748619028159)
--(axis cs:28,98.7634528596947)
--(axis cs:29,98.951689898847)
--(axis cs:30,99.1100658388061)
--(axis cs:31,99.1373788158105)
--(axis cs:32,99.2295452322118)
--(axis cs:33,99.3739885039028)
--(axis cs:34,99.5091437242361)
--(axis cs:35,99.5588971292252)
--(axis cs:36,99.6537155009335)
--(axis cs:37,99.6956961812455)
--(axis cs:38,99.6443514701181)
--(axis cs:39,99.7066108820709)
--(axis cs:40,99.7439665292425)
--(axis cs:41,99.7563799175455)
--(axis cs:42,99.7838279505273)
--(axis cs:43,99.8171305224128)
--(axis cs:44,99.801288518592)
--(axis cs:45,99.8049473542057)
--(axis cs:46,99.8384735150956)
--(axis cs:47,99.8530841090573)
--(axis cs:48,99.8618504654344)
--(axis cs:49,99.8871102792606)
--(axis cs:50,99.9122661675564)
--(axis cs:51,99.8888186808713)
--(axis cs:52,99.878796311095)
--(axis cs:53,99.897277786657)
--(axis cs:54,99.8798256523317)
--(axis cs:55,99.8899825129242)
--(axis cs:56,99.9339895077545)
--(axis cs:57,99.9403937046527)
--(axis cs:58,99.9342362227916)
--(axis cs:59,99.9135261124878)
--(axis cs:60,99.9481156674927)
--(axis cs:61,99.9488694004956)
--(axis cs:62,99.9161553923938)
--(axis cs:63,99.9296932354363)
--(axis cs:64,99.9578159412618)
--(axis cs:65,99.9546895647571)
--(axis cs:66,99.9728137388542)
--(axis cs:67,99.9536882433125)
--(axis cs:68,99.9522129459875)
--(axis cs:69,99.9513277675925)
--(axis cs:70,99.9707966605555)
--(axis cs:71,99.9624779963333)
--(axis cs:72,99.9474867978)
--(axis cs:73,99.96849207868)
--(axis cs:74,99.9431823687332)
--(axis cs:75,99.9659094212399)
--(axis cs:76,99.949545652744)
--(axis cs:77,99.9497273916464)
--(axis cs:78,99.9498364349878)
--(axis cs:79,99.9499018609927)
--(axis cs:80,99.9229254954085)
--(axis cs:81,99.9337552972451)
--(axis cs:82,99.940253178347)
--(axis cs:83,99.9641519070082)
--(axis cs:84,99.9784911442049)
--(axis cs:85,99.967094686523)
--(axis cs:86,99.9802568119138)
--(axis cs:87,99.9881540871482)
--(axis cs:88,99.9928924522889)
--(axis cs:89,99.9757354713734)
--(axis cs:90,99.965441282824)
--(axis cs:91,99.9792647696944)
--(axis cs:92,99.9875588618167)
--(axis cs:93,99.96253531709)
--(axis cs:94,99.957521190254)
--(axis cs:95,99.9545127141524)
--(axis cs:96,99.9527076284914)
--(axis cs:97,99.9716245770949)
--(axis cs:98,99.9829747462569)
--(axis cs:98,100.008123040023)
--(axis cs:98,100.008123040023)
--(axis cs:97,100.013538400038)
--(axis cs:96,100.022564000064)
--(axis cs:95,100.020940000107)
--(axis cs:94,100.018233333511)
--(axis cs:93,100.013722222519)
--(axis cs:92,100.006203704198)
--(axis cs:91,100.010339506997)
--(axis cs:90,100.017232511662)
--(axis cs:89,100.012054186103)
--(axis cs:88,100.003423643505)
--(axis cs:87,100.005706072508)
--(axis cs:86,100.009510120846)
--(axis cs:85,100.015850201411)
--(axis cs:84,100.009750335684)
--(axis cs:83,100.016250559474)
--(axis cs:82,100.02708426579)
--(axis cs:81,100.028473776317)
--(axis cs:80,100.030789627195)
--(axis cs:79,100.022956676679)
--(axis cs:78,100.021594461132)
--(axis cs:77,100.019324101887)
--(axis cs:76,100.015540169812)
--(axis cs:75,100.009233616354)
--(axis cs:74,100.01538936059)
--(axis cs:73,100.012460803525)
--(axis cs:72,100.020768005876)
--(axis cs:71,100.01794667646)
--(axis cs:70,100.013244460766)
--(axis cs:69,100.022074101277)
--(axis cs:68,100.020123502128)
--(axis cs:67,100.016872503547)
--(axis cs:66,100.011454172579)
--(axis cs:65,100.019090287631)
--(axis cs:64,100.015150479386)
--(axis cs:63,100.025250798976)
--(axis cs:62,100.025417998294)
--(axis cs:61,100.020419583984)
--(axis cs:60,100.017365973306)
--(axis cs:59,100.028943288844)
--(axis cs:58,100.019879446094)
--(axis cs:57,100.016465743491)
--(axis cs:56,100.010776239151)
--(axis cs:55,100.017960398586)
--(axis cs:54,100.016745866851)
--(axis cs:53,100.013674745314)
--(axis cs:52,100.006124575524)
--(axis cs:51,100.019382796827)
--(axis cs:50,100.018069628608)
--(axis cs:49,100.013449381013)
--(axis cs:48,100.005748968355)
--(axis cs:47,100.009581613925)
--(axis cs:46,100.015969356542)
--(axis cs:45,100.019124098524)
--(axis cs:44,100.005497235957)
--(axis cs:43,99.9941790685022)
--(axis cs:42,99.9683547009977)
--(axis cs:41,99.9639245016628)
--(axis cs:40,99.9732075027714)
--(axis cs:39,99.9720125046189)
--(axis cs:38,99.9700208410315)
--(axis cs:37,99.9615910040039)
--(axis cs:36,99.9584298078156)
--(axis cs:35,99.9613450520231)
--(axis cs:34,99.9412599111779)
--(axis cs:33,99.9266842217872)
--(axis cs:32,99.9215759772715)
--(axis cs:31,99.8811565333284)
--(axis cs:30,99.854159743092)
--(axis cs:29,99.8386860709832)
--(axis cs:28,99.7871737566889)
--(axis cs:27,99.7095157911568)
--(axis cs:26,99.6473486921144)
--(axis cs:25,99.5581717417973)
--(axis cs:24,99.4569352668048)
--(axis cs:23,99.3720235244429)
--(axis cs:22,99.170883630819)
--(axis cs:21,98.9301156980106)
--(axis cs:20,98.5909520105118)
--(axis cs:19,98.2025563324001)
--(axis cs:18,97.9974307357847)
--(axis cs:17,97.5188632521942)
--(axis cs:16,96.9093561270709)
--(axis cs:15,96.0523843826905)
--(axis cs:14,95.2106110524072)
--(axis cs:13,94.1132238887417)
--(axis cs:12,92.7359859074308)
--(axis cs:11,91.0458076283351)
--(axis cs:10,89.3057002748525)
--(axis cs:9,86.6746050822497)
--(axis cs:8,83.8841208414694)
--(axis cs:7,80.4981937167229)
--(axis cs:6,76.56256702499)
--(axis cs:5,72.071015663753)
--(axis cs:4,67.8719862068218)
--(axis cs:3,63.625928846399)
--(axis cs:2,59.1543651171822)
--(axis cs:1,54.5352892137471)
--(axis cs:0,51.8753730927767)
--cycle;

\addplot [semithick, color0]
table {%
0 76.0976616370068
1 76.5981796316751
2 75.7781308047139
3 73.3468698433429
4 68.3623167577677
5 64.2192633248083
6 59.0297217127178
7 52.3017195266863
8 45.9690282907919
9 40.6472631802213
10 34.8159215406581
11 30.2705472161403
12 26.1781747867799
13 22.691358222445
14 20.2185029227475
15 18.2352836223797
16 16.7604710083821
17 15.4259695896881
18 14.1658681697847
19 13.40972478496
20 12.5736987392025
21 11.842343484262
22 11.2631104999802
23 10.791394384794
24 10.504698940448
25 10.3457845359678
26 10.2312029027319
27 10.086706696117
28 9.88879617164486
29 9.8550844201543
30 9.75142919811517
31 9.71277623880767
32 9.72254942199002
33 9.66026385963324
34 9.87116939875489
35 9.91993326563119
36 9.80383781522561
37 9.77755799590228
38 9.7343121663933
39 9.57041415103753
40 9.55061225700138
41 9.57035945153357
42 9.57206943714222
43 9.66151090199342
44 9.71104040208854
45 9.77001280984878
46 9.70344104754673
47 9.66478431514779
48 9.75626382651337
49 9.75472675266684
50 9.78771254113257
51 9.80885256388657
52 9.7918171226676
53 9.94292609363471
54 10.158839730084
55 10.0682743244807
56 10.0253229723274
57 10.0276693311592
58 9.84506405341201
59 9.88734405779613
60 9.84712948994625
61 9.80835514891661
62 9.83227198124561
63 9.76217394638948
64 9.77519659935022
65 9.88997014690381
66 10.0085240501175
67 10.3534968669848
68 10.2258753829631
69 10.205538637996
70 10.1555837041461
71 10.409585182259
72 10.9127027617423
73 10.9471198994024
74 10.6971366725409
75 10.3926699094263
76 10.3333364491063
77 10.1502460330984
78 10.0310239143832
79 9.89209809659715
80 10.1037560387703
81 10.1300607382044
82 10.1823278061477
83 10.0926564796007
84 10.1682520278245
85 10.3367912943145
86 10.4544526057923
87 10.5002941017076
88 10.5905114377496
89 10.5640972699915
90 10.560818093884
91 10.4196722099547
92 10.7674815161798
93 11.0388251958993
94 10.7684287859852
95 10.6311098632708
96 10.8697010219099
97 10.9799498694221
98 10.7636639497439
};
\addlegendentry{non-targeted}
\addplot [semithick, color1]
table {%
0 50.2
1 52
2 55.36
3 58.991
4 62.7546
5 66.88776
6 71.092656
7 74.9205936
8 79.13235616
9 82.224413696
10 85.0346482176
11 87.45578893056
12 89.548473358336
13 91.1890840150016
14 92.483450409001
15 93.7400702454006
16 94.8240421472403
17 95.6044252883442
18 96.3876551730065
19 96.8075931038039
20 97.3245558622824
21 97.7797335173694
22 98.0528401104216
23 98.306704066253
24 98.5740224397518
25 98.8394134638511
26 98.9286480783106
27 99.1421888469864
28 99.2753133081918
29 99.3951879849151
30 99.4821127909491
31 99.5092676745694
32 99.5755606047417
33 99.650336362845
34 99.725201817707
35 99.7601210906242
36 99.8060726543745
37 99.8286435926247
38 99.8071861555748
39 99.8393116933449
40 99.8585870160069
41 99.8601522096042
42 99.8760913257625
43 99.9056547954575
44 99.9033928772745
45 99.9120357263647
46 99.9272214358188
47 99.9313328614913
48 99.9337997168948
49 99.9502798301369
50 99.9651678980821
51 99.9541007388493
52 99.9424604433096
53 99.9554762659857
54 99.9482857595914
55 99.9539714557549
56 99.9723828734529
57 99.9784297240718
58 99.9770578344431
59 99.9712347006658
60 99.9827408203995
61 99.9846444922397
62 99.9707866953438
63 99.9774720172063
64 99.9864832103238
65 99.9868899261943
66 99.9921339557166
67 99.9852803734299
68 99.986168224058
69 99.9867009344348
70 99.9920205606609
71 99.9902123363965
72 99.9841274018379
73 99.9904764411027
74 99.9792858646616
75 99.987571518797
76 99.9825429112782
77 99.9845257467669
78 99.9857154480601
79 99.9864292688361
80 99.9768575613017
81 99.981114536781
82 99.9836687220686
83 99.9902012332412
84 99.9941207399447
85 99.9914724439668
86 99.9948834663801
87 99.996930079828
88 99.9981580478968
89 99.9938948287381
90 99.9913368972429
91 99.9948021383457
92 99.9968812830074
93 99.9881287698044
94 99.9878772618827
95 99.9877263571296
96 99.9876358142778
97 99.9925814885667
98 99.99554889314
};
\addlegendentry{targeted}
\end{axis}

\end{tikzpicture}

==> figures/compare/compare_CartPole_vpg.tex <==
% This file was created by matplotlib2tikz v0.7.4.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.776470588235294,0.443137254901961,0.443137254901961}
\definecolor{color1}{rgb}{0.662745098039216,0.756862745098039,0.835294117647059}

\begin{axis}[
legend cell align={left},
legend style={draw=white!80.0!black},
tick align=outside,
tick pos=left,
title={CartPole,VPG,reward 0.3},
x grid style={white!69.01960784313725!black},
xlabel={Iterations},
xmin=-49.5, xmax=1039.5,
xtick style={color=black},
y grid style={white!69.01960784313725!black},
ylabel={Progress (\%)},
ymin=-15.9723491862867, ymax=126.184557114625,
ytick style={color=black}
]
\path [draw=color0, fill=color0, opacity=0.25]
(axis cs:0,63.1371596630135)
--(axis cs:0,28.1535322966138)
--(axis cs:10,26.8771957520405)
--(axis cs:20,22.5817448433229)
--(axis cs:30,19.7010852080942)
--(axis cs:40,15.661968387588)
--(axis cs:50,12.2398210367244)
--(axis cs:60,9.79538615456744)
--(axis cs:70,8.87435326509346)
--(axis cs:80,6.86247826486581)
--(axis cs:90,5.57828319855133)
--(axis cs:100,4.96818960026177)
--(axis cs:110,3.94143108094823)
--(axis cs:120,3.30687726398872)
--(axis cs:130,2.95144653719258)
--(axis cs:140,2.40802683200643)
--(axis cs:150,2.61480384851086)
--(axis cs:160,3.09628590777984)
--(axis cs:170,3.30093448657266)
--(axis cs:180,2.70773294923374)
--(axis cs:190,2.8245941621883)
--(axis cs:200,2.58441352541283)
--(axis cs:210,1.62543459568888)
--(axis cs:220,1.02782781129351)
--(axis cs:230,0.487906551319678)
--(axis cs:240,1.27558047326201)
--(axis cs:250,1.70942351730323)
--(axis cs:260,1.40694714344785)
--(axis cs:270,1.14336366394171)
--(axis cs:280,1.44830764891978)
--(axis cs:290,1.41954326495675)
--(axis cs:300,1.46424892991367)
--(axis cs:310,1.35343148306077)
--(axis cs:320,0.721924766938738)
--(axis cs:330,0.339204957232)
--(axis cs:340,-0.104025698824917)
--(axis cs:350,-1.03941991235672)
--(axis cs:360,-1.11793203205875)
--(axis cs:370,-1.18037274452837)
--(axis cs:380,-0.967035624482486)
--(axis cs:390,-0.959924666025333)
--(axis cs:400,-0.826389907208954)
--(axis cs:410,-0.853616084524977)
--(axis cs:420,-0.805970424899656)
--(axis cs:430,-1.11162646657302)
--(axis cs:440,-0.896034726229084)
--(axis cs:450,-0.784744015380125)
--(axis cs:460,-0.422341093678016)
--(axis cs:470,-0.48884651507545)
--(axis cs:480,-0.481574695180242)
--(axis cs:490,-0.349493651971075)
--(axis cs:500,-0.400452576876972)
--(axis cs:510,-0.497730339369221)
--(axis cs:520,-0.35488624726865)
--(axis cs:530,-0.00692032591503139)
--(axis cs:540,0.278720083105979)
--(axis cs:550,0.616178061652232)
--(axis cs:560,1.08021094144396)
--(axis cs:570,1.52174572158186)
--(axis cs:580,1.81990397935015)
--(axis cs:590,1.83919806698179)
--(axis cs:600,2.10089751369919)
--(axis cs:610,2.29151144700693)
--(axis cs:620,1.91959268438038)
--(axis cs:630,1.2293289890215)
--(axis cs:640,0.83167802955629)
--(axis cs:650,0.22574411477726)
--(axis cs:660,-0.317661469009813)
--(axis cs:670,-0.556167848052432)
--(axis cs:680,-1.07649732420583)
--(axis cs:690,-0.881596969650558)
--(axis cs:700,-0.801530142961402)
--(axis cs:710,-0.542886622799372)
--(axis cs:720,-0.589043897009563)
--(axis cs:730,-0.478359236054307)
--(axis cs:740,-0.73906253738559)
--(axis cs:750,-0.888386719504456)
--(axis cs:760,-0.678969551565645)
--(axis cs:770,-0.718639339169102)
--(axis cs:780,-0.965915837858293)
--(axis cs:790,-1.25014401224769)
--(axis cs:800,-1.79822738562417)
--(axis cs:810,-2.38397046105468)
--(axis cs:820,-2.99111071449551)
--(axis cs:830,-3.66618390370942)
--(axis cs:840,-4.35719995511317)
--(axis cs:850,-5.15610301121538)
--(axis cs:860,-4.95263444313755)
--(axis cs:870,-5.68208229593766)
--(axis cs:880,-5.50541068484348)
--(axis cs:890,-5.85879656032723)
--(axis cs:900,-6.1822866947906)
--(axis cs:910,-6.81611830530142)
--(axis cs:920,-7.97117119539393)
--(axis cs:930,-9.10249709784539)
--(axis cs:940,-9.51067162715431)
--(axis cs:950,-9.15348400465829)
--(axis cs:960,-8.9367088761241)
--(axis cs:970,-8.91155494464763)
--(axis cs:980,-8.72272694019626)
--(axis cs:990,-8.58413449881924)
--(axis cs:990,34.1572924876351)
--(axis cs:990,34.1572924876351)
--(axis cs:980,34.1812949135164)
--(axis cs:970,34.3646386923674)
--(axis cs:960,34.40809488133)
--(axis cs:950,34.6929713028577)
--(axis cs:940,35.2977413135745)
--(axis cs:930,34.9982508814848)
--(axis cs:920,34.0545927312824)
--(axis cs:910,33.5000242817001)
--(axis cs:900,33.0470040100832)
--(axis cs:890,31.1943453935512)
--(axis cs:880,29.1310678132074)
--(axis cs:870,28.4233752966096)
--(axis cs:860,26.6902413420562)
--(axis cs:850,26.771192913264)
--(axis cs:840,25.3896410593843)
--(axis cs:830,24.340904558636)
--(axis cs:820,23.0296417984425)
--(axis cs:810,21.8172849890677)
--(axis cs:800,21.6107870947849)
--(axis cs:790,21.4321288187642)
--(axis cs:780,21.4888735867549)
--(axis cs:770,21.3526578675142)
--(axis cs:760,21.4309620792282)
--(axis cs:750,20.5832870813236)
--(axis cs:740,19.0914092559724)
--(axis cs:730,18.4665766735887)
--(axis cs:720,18.6050945873316)
--(axis cs:710,18.5144412708719)
--(axis cs:700,18.9027167316407)
--(axis cs:690,19.1687705346677)
--(axis cs:680,19.6269156454989)
--(axis cs:670,19.0419800848268)
--(axis cs:660,18.9170622129561)
--(axis cs:650,18.3247600447333)
--(axis cs:640,18.1280622784027)
--(axis cs:630,18.276254133333)
--(axis cs:620,18.7134565423846)
--(axis cs:610,19.4486663072948)
--(axis cs:600,19.9591725609471)
--(axis cs:590,19.6580368834416)
--(axis cs:580,18.9352450584602)
--(axis cs:570,17.7486466985833)
--(axis cs:560,17.0010999403932)
--(axis cs:550,16.9450677093467)
--(axis cs:540,17.6902257255559)
--(axis cs:530,18.5405966027683)
--(axis cs:520,19.2587799947861)
--(axis cs:510,19.8064494947286)
--(axis cs:500,19.9361465117456)
--(axis cs:490,20.8743324449468)
--(axis cs:480,21.4294316524694)
--(axis cs:470,19.8543714941304)
--(axis cs:460,18.5331223220506)
--(axis cs:450,17.4804409984146)
--(axis cs:440,16.4709127311604)
--(axis cs:430,16.4468905871725)
--(axis cs:420,16.0721045566099)
--(axis cs:410,16.1674615438807)
--(axis cs:400,16.4451955912373)
--(axis cs:390,17.1480336432657)
--(axis cs:380,17.3491577957271)
--(axis cs:370,17.7090932452831)
--(axis cs:360,18.0390358623995)
--(axis cs:350,18.3520590274791)
--(axis cs:340,16.8549434268696)
--(axis cs:330,16.408777778117)
--(axis cs:320,15.9662438744936)
--(axis cs:310,14.5889988077445)
--(axis cs:300,14.4123127223031)
--(axis cs:290,15.1119681517205)
--(axis cs:280,15.3943172493377)
--(axis cs:270,15.1728967374812)
--(axis cs:260,12.7154325437745)
--(axis cs:250,12.5988636384968)
--(axis cs:240,14.9898924345414)
--(axis cs:230,18.8801159781216)
--(axis cs:220,19.5979849194204)
--(axis cs:210,19.5745369154557)
--(axis cs:200,17.303501905175)
--(axis cs:190,18.1662043059888)
--(axis cs:180,20.6001395207244)
--(axis cs:170,21.3922339283146)
--(axis cs:160,23.2667204134762)
--(axis cs:150,26.5331516686008)
--(axis cs:140,27.8320448277137)
--(axis cs:130,28.0801444701754)
--(axis cs:120,28.7698308628767)
--(axis cs:110,28.117095262448)
--(axis cs:100,29.2335195444998)
--(axis cs:90,32.4545717467854)
--(axis cs:80,33.5159025097067)
--(axis cs:70,35.3259178379208)
--(axis cs:60,38.7028789633889)
--(axis cs:50,41.6212017448295)
--(axis cs:40,47.5968659630288)
--(axis cs:30,51.8247564860549)
--(axis cs:20,56.9353333413178)
--(axis cs:10,60.8133567427469)
--(axis cs:0,63.1371596630135)
--cycle;

\path [draw=color1, fill=color1, opacity=0.25]
(axis cs:0,73.5692073511655)
--(axis cs:0,40.870897576248)
--(axis cs:10,42.7793346000079)
--(axis cs:20,45.0008224148875)
--(axis cs:30,46.511303761428)
--(axis cs:40,46.8900581243948)
--(axis cs:50,47.4792638617031)
--(axis cs:60,46.695664394198)
--(axis cs:70,46.1403884369505)
--(axis cs:80,45.2382230606631)
--(axis cs:90,44.5073171165847)
--(axis cs:100,44.0008686849685)
--(axis cs:110,43.1938774977482)
--(axis cs:120,42.7691092810411)
--(axis cs:130,41.8918553881104)
--(axis cs:140,40.736269571442)
--(axis cs:150,40.3017618352621)
--(axis cs:160,39.7378330314989)
--(axis cs:170,39.4698535054881)
--(axis cs:180,39.2652208376279)
--(axis cs:190,39.0511313807863)
--(axis cs:200,39.2054997491749)
--(axis cs:210,38.9293614794015)
--(axis cs:220,39.0047427688038)
--(axis cs:230,39.5658552187274)
--(axis cs:240,39.8797049634143)
--(axis cs:250,40.0500417327039)
--(axis cs:260,40.9045401506191)
--(axis cs:270,41.6121941948416)
--(axis cs:280,41.3962903363076)
--(axis cs:290,41.2790232130047)
--(axis cs:300,40.7988480372443)
--(axis cs:310,40.719475917173)
--(axis cs:320,40.7853987809722)
--(axis cs:330,40.7492843591477)
--(axis cs:340,40.4507921905594)
--(axis cs:350,40.4202637427786)
--(axis cs:360,40.2206213367855)
--(axis cs:370,40.5751584866015)
--(axis cs:380,40.8390486341006)
--(axis cs:390,41.5296895028688)
--(axis cs:400,42.0687884746361)
--(axis cs:410,42.2097069553799)
--(axis cs:420,42.0624524217151)
--(axis cs:430,41.9953369794576)
--(axis cs:440,42.1418389589325)
--(axis cs:450,42.0301176710681)
--(axis cs:460,42.2482105408344)
--(axis cs:470,42.726006197949)
--(axis cs:480,42.9067550506221)
--(axis cs:490,43.3223010020227)
--(axis cs:500,43.9883578042133)
--(axis cs:510,44.4212897588293)
--(axis cs:520,44.5687318615789)
--(axis cs:530,44.94953859776)
--(axis cs:540,45.5474788344426)
--(axis cs:550,45.8841145932513)
--(axis cs:560,46.4284238550807)
--(axis cs:570,47.0515925644349)
--(axis cs:580,47.3142462313254)
--(axis cs:590,47.8277232372978)
--(axis cs:600,48.5006127536769)
--(axis cs:610,48.8322779510031)
--(axis cs:620,49.0359891227795)
--(axis cs:630,49.5744933759032)
--(axis cs:640,50.1758563578744)
--(axis cs:650,50.2772902134172)
--(axis cs:660,51.1851161400713)
--(axis cs:670,52.7398675590165)
--(axis cs:680,53.6181443055862)
--(axis cs:690,55.1098668547006)
--(axis cs:700,55.7967337278286)
--(axis cs:710,57.0375922342307)
--(axis cs:720,57.8967778099123)
--(axis cs:730,58.8824325666079)
--(axis cs:740,59.0451493354256)
--(axis cs:750,60.3502875783148)
--(axis cs:760,60.9156661124517)
--(axis cs:770,61.4878239051839)
--(axis cs:780,62.2227535704505)
--(axis cs:790,62.6144140517737)
--(axis cs:800,62.8327663989387)
--(axis cs:810,63.4588985888715)
--(axis cs:820,63.6007506297692)
--(axis cs:830,63.9714892400356)
--(axis cs:840,64.565588031058)
--(axis cs:850,65.359922631046)
--(axis cs:860,65.4312963095491)
--(axis cs:870,66.3141066293007)
--(axis cs:880,66.5119662268048)
--(axis cs:890,67.1974438866665)
--(axis cs:900,68.1714380577455)
--(axis cs:910,68.1606678690472)
--(axis cs:920,69.234415704547)
--(axis cs:930,70.2395473724975)
--(axis cs:940,70.8442715078871)
--(axis cs:950,71.0035946219499)
--(axis cs:960,71.3156344408727)
--(axis cs:970,71.5035100702007)
--(axis cs:980,71.7376567757016)
--(axis cs:990,72.3647042095238)
--(axis cs:990,119.722879555493)
--(axis cs:990,119.722879555493)
--(axis cs:980,119.229630690248)
--(axis cs:970,119.411874446773)
--(axis cs:960,119.18363658383)
--(axis cs:950,118.885087231809)
--(axis cs:940,118.799248967253)
--(axis cs:930,118.719128388878)
--(axis cs:920,118.219395105183)
--(axis cs:910,117.771692861719)
--(axis cs:900,117.531351709864)
--(axis cs:890,117.153309473562)
--(axis cs:880,116.918865781093)
--(axis cs:870,116.560129895797)
--(axis cs:860,115.817784813873)
--(axis cs:850,115.862240463669)
--(axis cs:840,115.679031527025)
--(axis cs:830,115.314570976772)
--(axis cs:820,114.940011497724)
--(axis cs:810,114.0892732445)
--(axis cs:800,113.758808479843)
--(axis cs:790,113.265321974265)
--(axis cs:780,112.858781865231)
--(axis cs:770,111.967405974581)
--(axis cs:760,111.756182187778)
--(axis cs:750,110.54909764615)
--(axis cs:740,109.107614825602)
--(axis cs:730,108.487838942964)
--(axis cs:720,107.208262398837)
--(axis cs:710,105.949167003594)
--(axis cs:700,104.71396368034)
--(axis cs:690,104.118547154322)
--(axis cs:680,102.785517492698)
--(axis cs:670,101.929873619486)
--(axis cs:660,101.732044945118)
--(axis cs:650,101.072450220493)
--(axis cs:640,100.762723042374)
--(axis cs:630,100.289883689749)
--(axis cs:620,100.366533147828)
--(axis cs:610,99.9119016254855)
--(axis cs:600,100.047866751308)
--(axis cs:590,99.6374498800622)
--(axis cs:580,99.2352391069231)
--(axis cs:570,98.9456365745691)
--(axis cs:560,98.9320127357694)
--(axis cs:550,98.5010185135038)
--(axis cs:540,98.082769112988)
--(axis cs:530,97.4896912603989)
--(axis cs:520,97.3521913074036)
--(axis cs:510,97.501636016056)
--(axis cs:500,97.2955618845639)
--(axis cs:490,97.2070556773058)
--(axis cs:480,96.7122794848018)
--(axis cs:470,96.0901025574575)
--(axis cs:460,94.9675955151498)
--(axis cs:450,93.8809700484932)
--(axis cs:440,93.4166417591502)
--(axis cs:430,93.1089882445697)
--(axis cs:420,91.9363246031816)
--(axis cs:410,91.4832496268493)
--(axis cs:400,90.5340207420908)
--(axis cs:390,90.0929928594804)
--(axis cs:380,89.6645145298584)
--(axis cs:370,88.988951673641)
--(axis cs:360,88.5885144428645)
--(axis cs:350,87.6263564994672)
--(axis cs:340,87.0990178025505)
--(axis cs:330,86.9018758183944)
--(axis cs:320,85.9860939626991)
--(axis cs:310,85.2173347182728)
--(axis cs:300,84.8588501340806)
--(axis cs:290,84.01333876203)
--(axis cs:280,83.628248832687)
--(axis cs:270,82.6627290339752)
--(axis cs:260,81.3629708077087)
--(axis cs:250,80.8414933429623)
--(axis cs:240,80.5458729829192)
--(axis cs:230,80.1283822519718)
--(axis cs:220,79.9054551545918)
--(axis cs:210,79.171002677269)
--(axis cs:200,78.8672250182295)
--(axis cs:190,78.3351414167074)
--(axis cs:180,78.4468800819913)
--(axis cs:170,77.7374673856265)
--(axis cs:160,76.8870587856099)
--(axis cs:150,76.3169826508646)
--(axis cs:140,76.4923852074156)
--(axis cs:130,76.1744708681576)
--(axis cs:120,75.8294770044515)
--(axis cs:110,75.0519749978095)
--(axis cs:100,74.4173144689568)
--(axis cs:90,74.2571758349912)
--(axis cs:80,73.1686729795667)
--(axis cs:70,73.6002995058486)
--(axis cs:60,72.9134664631094)
--(axis cs:50,72.9785080094279)
--(axis cs:40,74.3284984335488)
--(axis cs:30,75.1072823296577)
--(axis cs:20,75.65143378439)
--(axis cs:10,74.4590078194479)
--(axis cs:0,73.5692073511655)
--cycle;

\addplot [semithick, color0]
table {%
0 45.6453459798136
10 43.8452762473937
20 39.7585390923203
30 35.7629208470745
40 31.6294171753084
50 26.9305113907769
60 24.2491325589781
70 22.1001355515071
80 20.1891903872863
90 19.0164274726684
100 17.1008545723808
110 16.0292631716981
120 16.0383540634327
130 15.515795503684
140 15.12003582986
150 14.5739777585558
160 13.181503160628
170 12.3465842074437
180 11.6539362349791
190 10.4953992340885
200 9.94395771529392
210 10.5999857555723
220 10.312906365357
230 9.68401126472063
240 8.13273645390172
250 7.1541435779
260 7.06118984361119
270 8.15813020071144
280 8.42131244912873
290 8.26575570833864
300 7.9382808261084
310 7.97121514540262
320 8.34408432071619
330 8.37399136767451
340 8.37545886402235
350 8.6563195575612
360 8.46055191517038
370 8.26436025037738
380 8.19106108562232
390 8.0940544886202
400 7.80940284201418
410 7.65692272967785
420 7.6330670658551
430 7.66763206029972
440 7.78743900246564
450 8.34784849151721
460 9.05539061418628
470 9.68276248952748
480 10.4739284786446
490 10.2624193964879
500 9.76784696743431
510 9.65435957767968
520 9.45194687375874
530 9.26683813842665
540 8.98447290433094
550 8.78062288549945
560 9.0406554409186
570 9.63519621008256
580 10.3775745189052
590 10.7486174752117
600 11.0300350373231
610 10.8700888771509
620 10.3165246133825
630 9.75279156117723
640 9.47987015397952
650 9.27525207975529
660 9.29970037197317
670 9.2429061183872
680 9.27520916064655
690 9.14358678250855
700 9.05059329433965
710 8.98577732403624
720 9.00802534516103
730 8.99410871876722
740 9.17617335929343
750 9.84745018090958
760 10.3759962638313
770 10.3170092641726
780 10.2614788744483
790 10.0909924032582
800 9.90627985458035
810 9.71665726400653
820 10.0192655419735
830 10.3373603274633
840 10.5162205521356
850 10.8075449510243
860 10.8688034494593
870 11.370646500336
880 11.812828564182
890 12.667774416612
900 13.4323586576463
910 13.3419529881993
920 13.0417107679443
930 12.9478768918197
940 12.8935348432101
950 12.7697436490997
960 12.735693002603
970 12.7265418738599
980 12.7292839866601
990 12.7865789944079
};
\addlegendentry{non-targeted}
\addplot [semithick, color1]
table {%
0 57.2200524637068
10 58.6191712097279
20 60.3261280996388
30 60.8092930455429
40 60.6092782789718
50 60.2288859355655
60 59.8045654286537
70 59.8703439713995
80 59.2034480201149
90 59.382246475788
100 59.2090915769626
110 59.1229262477789
120 59.2992931427463
130 59.033163128134
140 58.6143273894288
150 58.3093722430634
160 58.3124459085544
170 58.6036604455573
180 58.8560504598096
190 58.6931363987468
200 59.0363623837022
210 59.0501820783353
220 59.4550989616978
230 59.8471187353496
240 60.2127889731668
250 60.4457675378331
260 61.1337554791639
270 62.1374616144084
280 62.5122695844973
290 62.6461809875173
300 62.8288490856624
310 62.9684053177229
320 63.3857463718357
330 63.8255800887711
340 63.7749049965549
350 64.0233101211229
360 64.404567889825
370 64.7820550801212
380 65.2517815819795
390 65.8113411811746
400 66.3014046083635
410 66.8464782911146
420 66.9993885124484
430 67.5521626120137
440 67.7792403590413
450 67.9555438597806
460 68.6079030279921
470 69.4080543777033
480 69.8095172677119
490 70.2646783396643
500 70.6419598443886
510 70.9614628874426
520 70.9604615844912
530 71.2196149290795
540 71.8151239737153
550 72.1925665533775
560 72.6802182954251
570 72.998614569502
580 73.2747426691243
590 73.73258655868
600 74.2742397524925
610 74.3720897882443
620 74.7012611353037
630 74.9321885328259
640 75.4692897001243
650 75.6748702169549
660 76.4585805425949
670 77.3348705892514
680 78.2018308991421
690 79.6142070045111
700 80.2553487040842
710 81.4933796189123
720 82.5525201043745
730 83.685135754786
740 84.0763820805137
750 85.4496926122326
760 86.3359241501149
770 86.7276149398822
780 87.5407677178407
790 87.9398680130193
800 88.2957874393908
810 88.774085916686
820 89.2703810637467
830 89.6430301084038
840 90.1223097790415
850 90.6110815473575
860 90.6245405617112
870 91.4371182625487
880 91.7154160039489
890 92.1753766801141
900 92.8513948838045
910 92.9661803653832
920 93.726905404865
930 94.479337880688
940 94.8217602375703
950 94.9443409268796
960 95.2496355123513
970 95.4576922584867
980 95.4836437329749
990 96.0437918825082
};
\addlegendentry{targeted}
\end{axis}

\end{tikzpicture}

==> include/talks/supp_macros.tex <==
\definecolor{mygray}{gray}{0.6}
\newcommand{\mycite}[1]{\textcolor{mygray}{\scriptsize{#1}}}

%\newcommand{\myvector}[1]{\ensuremath{\bm{#1}}}
%\newcommand{\mymatrix}[1]{\ensuremath{\bm{#1}}}
%\newcommand{\mytensor}[1]{\bm{\mathcal{#1}}}
%\newcommand{\tensor}[1]{\bm{\mathcal{#1}}}
\newcommand\Dir{\operatorname{Dir}}
\def\tl{\tilde}

\renewcommand\t{{\scriptscriptstyle\top}}

\newcommand\iideq{\stackrel{\mathclap{\normalfont\mbox{\scriptsize{iid}}}}{=}}
\newcommand\iidsim{\stackrel{\mathclap{\normalfont\mbox{\scriptsize{iid}}}}{\sim}}
\newcommand\aseq{\stackrel{\mathclap{\normalfont\mbox{\scriptsize{a.s.}}}}{=}}
\newcommand\whpeq{\stackrel{\mathclap{\normalfont\mbox{\scriptsize{w.h.p.}}}}{\ =\ }}



%\newcommand{\vectorSub}[2]{\ensuremath{\bm{#1}}_{#2}}	
%\newcommand{\vectorSup}[2]{\ensuremath{\bm{#1}}^{(#2)}}
%\newcommand{\vectorInd}[3]{\ensuremath{\bm{#1}}_{#2}^{(#3)}}
%\newcommand{\matrixSub}[2]{\ensuremath{\bm{#1}}_{#2}}	
%\newcommand{\matrixSup}[2]{\ensuremath{\bm{#1}}^{(#2)}}
%\newcommand{\matrixInd}[3]{\ensuremath{\bm{#1}}_{#2}^{(#3)}}
%\newcommand{\tensorSub}[2]{\ensuremath{\bm{\mathcal{#1}}}_{#2}}	
%\newcommand{\tensorSup}[2]{\ensuremath{\bm{\mathcal{#1}}}^{(#2)}}
%\newcommand{\tensorInd}[3]{\ensuremath{\bm{\mathcal{#1}}}_{#2}^{(#3)}}

%\newcommand{\swapaxes}{\mathsf{swapaxes}}
%\newcommand{\flipaxis}{\mathsf{flipaxis}}

%\newcommand\cpeq{\mathrel{\stackrel{\makebox[0pt]{\mbox{\normalfont\tiny cp}}}{=}}}
%\newcommand\tkeq{\mathrel{\stackrel{\makebox[0pt]{\mbox{\normalfont\tiny tk}}}{=}}}
%\newcommand\tteq{\mathrel{\stackrel{\makebox[0pt]{\mbox{\normalfont\tiny tt}}}{=}}}


\newcommand\asymptoticeq{\stackrel{\mathclap{\normalfont\mbox{\scriptsize{\ensuremath{n\!\!\rightarrow\!\!\infty}}}}}{\quad =\quad }}

\newcommand{\mle}{\ensuremath{{\mathsf{mle}}}}
\DeclareMathOperator{\Triples}{T}
\newcommand\inner[1]{\ensuremath{\langle #1 \rangle}}
 \def\hC{\widehat{C}}
\def\hE{\widehat{E}}
% \def\hF{\widehat{F}}
 \def\hG{\widehat{G}}
  \def\hG{\widehat{J}}
 \def\hk{\widehat{k}}
\def\hl{\widehat{l}}
 \def\hSigma{{\widehat{\Sigma}}}
\DeclareMathOperator{\poly}{poly}

 \def\0{{\bf 0}}

\def\leqst{{\overset{st}{\leq}}}
\def\geqst{{\overset{st}{\geq}}}
\def\geqrh{{\overset{rh}{\geq}}}
\def\geqlr{{\overset{lr}{\geq}}}
\def\eqlr{{\overset{lr}{=}}}
\DeclarePairedDelimiter\norm{\lVert}{\rVert}
\DeclareMathOperator{\atanh}{atanh}
\def\tilomega{{\widetilde{\omega}}}
\def\edoc{\end{document}}

\DeclareMathOperator{\rank}{Rank}
  \DeclareMathOperator{\tw}{tw}
\def\Tsawi{{T_{\mathrm{saw}}(i;G)}}
\DeclareMathOperator{\Deg}{Deg}
\DeclareMathOperator{\aug}{Aug}
\DeclareMathOperator{\watts}{Watts}
\DeclareMathOperator{\girth}{Girth}
\DeclareMathOperator{\PL}{PL}
\DeclareMathOperator{\LP}{LP}
\DeclareMathOperator{\ER}{ER}
\DeclareMathOperator{\reg}{Reg}
%mbox - function definitions
\def\tha{\mbox{\tiny th}}
\DeclareMathOperator{\Det}{Det}
\newcommand{\Var}{\mbox{Var}}
\newcommand{\Cov}{\mbox{Cov}}
\newcommand{\Poiss}{\mbox{${\mbox{Poiss}}$}}
\newcommand{\Diag}{\mbox{${\mbox{Diag}}$}}
\newcommand{\Diam}{\mbox{${\mbox{Diam}}$}}
\def\erf{\mbox{erf}}
\def\erfc{\mbox{erfc}}
\def\qfunc{\mbox{Q}}
\def\myexp{\mbox{e}}
\def\snr{\mbox{\tiny SNR}}
\def\signum{\mbox{sgn}}
\def\Card{\mbox{\small N}}
\def\plim{\mbox{p\,}\lim}
\def\convd{\overset{d}\rightarrow}
\def\convp{\overset{p}\rightarrow}
\newcommand\indep{\protect\mathpalette{\protect\independenT}{\perp}}
\def\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern2mu{#1#2}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%text abbreviations
\def\etal{{et al. \/}}
\def\viz{{viz.,\ \/}}
\def\ie{{i.e.,\ \/}}
\def\eg{{e.g.,  }}
\def\etc{{etc.,  }}
\def\ifff{{iff  }}
\def\as{{a.s.  }}
\def\st{{s.t.  }}
\def\wpone{{w.p.}\,1\,\,}
\def\nn{\nonumber}
\def\qed{\hfill$\Box$}
\def\complx{\mathbb{C}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% LDP
%
%\def\EGnp{\tilde{E}^{\mbox{\tiny NPD}}(\lambda)}
%\def\EGB{\tilde{E}^{\mbox{\tiny BD}}(\lambda)}
%\def\EGFI{\tilde{E}^{\mbox{\tiny MLE}}(\lambda,\theta)}
%\def\trueEGnp{{E}^{\mbox{\tiny NPD}}(\lambda)}
%\def\trueEGB{{E}^{\mbox{\tiny BD}}(\lambda)}
%\def\trueEFI{{E}^{\mbox{\tiny MLE}}(\lambda,\theta)}
%\def\thetaml{\hat{\theta}_{{\mbox{\tiny MLE}}}}
%\def\nustar{\nu_{*}}
%\def\trueEB{{E}^{\mbox{\tiny D}}(\lambdabf)}
%\def\trueEF{{E}^{\mbox{\tiny E}}(\lambdabf)}
%\def\tilDlambdagamma{\tilde{D}_{\lambda,\gamma}}
%\def\tilClambdagamma{\tilde{C}_{\lambda,\gamma}}
%\def\tilD{\tilde{D}}
%\def\tilC{\tilde{C}}
%\def\delpj{\Delta p_\theta(j)}
%\def\mindet{\hat{\theta}_{\mbox{\tiny mrd}}}
%\def\minsumrate{\hat{\theta}_{\mbox{\tiny msd}}}
%\def\sprt{\mathbb{E}_{\theta_i}N_{\mbox{\tiny sprt}}(\lambda)}
%\def\smst{\mathbb{E}_{\theta_i}N_{\mbox{\tiny smst}}(\lambda)}
%\def\sprtzero{\mathbb{E}_{\theta_0}N_{\mbox{\tiny sprt}}(\lambda)}
%\def\smstzero{\mathbb{E}_{\theta_0}N_{\mbox{\tiny smst}}(\lambda)}
%\def\sprtone{\mathbb{E}_{\theta_1}N_{\mbox{\tiny sprt}}(\lambda)}
%\def\smstone{\mathbb{E}_{\theta_1}N_{\mbox{\tiny smst}}(\lambda)}
%\def\nsprt{N_{\mbox{\tiny sprt}}}
%\def\nsmst{N_{\mbox{\tiny smst}}}
%\def\diffseq{\mathbb{E}_{\theta_i}(N_{\mbox{\tiny sprt}}-N_{\mbox{\tiny
%smst}})(\lambda)}
%\def\xij{\{X_{i,j}\}}
%\def\xioneseq{\{X_{i,1}\}_{i=1}^\infty}
%\def\xinseq{\{X_{i,n}\}_{i=1}^\infty}
%\def\xij{X_{i,j}}
%\def\hione{H_{i,1}}
%\def\hitwo{H_{i,2}}
%\def\hij{H_{i,j}}
%\def\snrt{\mbox{\scriptsize{SNR}}_t}
%\def\snrr{\mbox{\small{SNR}}_r}
%\def\plim{\mbox{p}\lim}
%\def\convd{\overset{d}\rightarrow}
%\def\convp{\overset{p}\rightarrow}
%\def\convweak{\Rightarrow}
%%\def\bfptheta{\mathbf{p}_{\theta}}
%\def\pt{\mathbf{p}_{\theta}}
%\def\pti{\mathbf{p}_{\theta_i}}
%\def\ptzero{\mathbf{p}_{\theta_0}}
%\def\ptone{\mathbf{p}_{\theta_1}}
%\def\pthetai{p_{\theta_i}}
%\def\ptheta{p_{\theta}}
%\def\conv{{ \rightarrow}}
%\def\balle{\mathcal{B}_\epsilon}
%\def\thetai{\theta_i}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%presentation specs
\def\tcr{\textcolor{red}}
\def\tcb{\textcolor{blue}}
\def\tcg{\textcolor{green}}
\def\tcw{\textcolor{white}}
\def\tcm{\textcolor{magenta}}
\def\tccyan{\textcolor{cyan}}
\def\tcv{\textcolor{violet}}
\definecolor{dkr}{rgb}{0.6,0.2,0.2}
\definecolor{dkg}{rgb}{0,0.5,0}
\definecolor{dkb}{rgb}{0.0,0.1,0.7}

\def\tcdkb{\textcolor{dkb}}
\def\tcdkg{\textcolor{dkg}}
\def\tcdkr{\textcolor{dkr}}
\def\tcblack{\textcolor{black}}

%beamer
\newcommand{\ft}{\frametitle}
\newcommand{\bef}{\begin{frame}}
\newcommand{\eef}{\end{frame}}%strange doesnt work
\newcommand{\beb}{\begin{block}}
\newcommand{\eeb}{\end{block}}
\newcommand{\becs}{\begin{columns}}
\newcommand{\eecs}{\end{columns}}
\newcommand{\bec}{\begin{column}}
\newcommand{\eec}{\end{column}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\mathscr

\newcommand{\Amsc}{\mathscr{A}}
\newcommand{\Cmsc}{\mathscr{C}}
\newcommand{\Dmsc}{\mathscr{D}}
\newcommand{\Emsc}{\mathscr{E}}
\newcommand{\Fmsc}{\mathscr{F}}
\newcommand{\Gmsc}{\mathscr{G}}
\newcommand{\Hmsc}{\mathscr{H}}
\newcommand{\Kmsc}{\mathscr{K}}
\newcommand{\Nmsc}{\mathscr{N}}
\newcommand{\Pmsc}{\mathscr{P}}
\newcommand{\Qmsc}{\mathscr{Q}}
\newcommand{\Rmsc}{\mathscr{R}}
\newcommand{\Smsc}{\mathscr{S}}
\newcommand{\Tmsc}{\mathscr{T}}
\newcommand{\Umsc}{\mathscr{U}}
\newcommand{\Xmsc}{\mathscr{X}}
\newcommand{\Ymsc}{\mathscr{Y}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%bold alphabets
\def\bfzero{{\mathbf{0}}}
\def\bfone{{\mathbf{1}}}
\def\bfa{{\mathbf a}}
\def\bfb{{\mathbf b}}
\def\bfc{{\mathbf c}}
\def\bfd{{\mathbf d}}
\def\bfe{{\mathbf e}}
\def\bff{{\mathbf f}}
\def\bfg{{\mathbf g}}
\def\bfh{{\mathbf h}}
\def\bfi{{\mathbf i}}
\def\bfj{{\mathbf j}}
\def\bfk{{\mathbf k}}
\def\bfl{{\mathbf l}}
\def\bfm{{\mathbf m}}
\def\bfn{{\mathbf n}}
\def\bfo{{\mathbf o}}
\def\bfp{{\mathbf p}}
\def\bfq{{\mathbf q}}
\def\bfr{{\mathbf r}}
\def\bfs{{\mathbf s}}
\def\bft{{\mathbf t}}
\def\bfu{{\mathbf u}}
\def\bfv{{\mathbf v}}
\def\bfw{{\mathbf w}}
\def\bfx{{\mathbf x}}
\def\bfy{{\mathbf y}}
\def\bfz{{\mathbf z}}
%bold caps
\def\bfA{{\mathbf A}}
\def\bfB{{\mathbf B}}
\def\bfC{{\mathbf C}}
\def\bfD{{\mathbf D}}
\def\bfE{{\mathbf E}}
\def\bfF{{\mathbf F}}
\def\bfG{{\mathbf G}}
\def\bfH{{\mathbf H}}
\def\bfI{{\mathbf I}}
\def\bfJ{{\mathbf J}}
\def\bfK{{\mathbf K}}
\def\bfL{{\mathbf L}}
\def\bfM{{\mathbf M}}
\def\bfN{{\mathbf N}}
\def\bfO{{\mathbf O}}
\def\bfP{{\mathbf P}}
\def\bfQ{{\mathbf Q}}
\def\bfR{{\mathbf R}}
\def\bfS{{\mathbf S}}
\def\bfT{{\mathbf T}}
\def\bfU{{\mathbf U}}
\def\bfV{{\mathbf V}}
\def\bfW{{\mathbf W}}
\def\bfX{{\mathbf X}}
\def\bfY{{\mathbf Y}}
\def\bfZ{{\mathbf Z}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%bold symbols

\def\alphabf{\hbox{\boldmath$\alpha$\unboldmath}}
\def\betabf{\hbox{\boldmath$\beta$\unboldmath}}
\def\gammabf{\hbox{\boldmath$\gamma$\unboldmath}}
\def\deltabf{\hbox{\boldmath$\delta$\unboldmath}}
\def\epsilonbf{\hbox{\boldmath$\epsilon$\unboldmath}}
\def\zetabf{\hbox{\boldmath$\zeta$\unboldmath}}
\def\etabf{\hbox{\boldmath$\eta$\unboldmath}}
\def\iotabf{\hbox{\boldmath$\iota$\unboldmath}}
\def\kappabf{\hbox{\boldmath$\kappa$\unboldmath}}
\def\lambdabf{\hbox{\boldmath$\lambda$\unboldmath}}
\def\mubf{\hbox{\boldmath$\mu$\unboldmath}}
\def\nubf{\hbox{\boldmath$\nu$\unboldmath}}
\def\xibf{\hbox{\boldmath$\xi$\unboldmath}}
\def\pibf{\hbox{\boldmath$\pi$\unboldmath}}
\def\rhobf{\hbox{\boldmath$\rho$\unboldmath}}
\def\sigmabf{\hbox{\boldmath$\sigma$\unboldmath}}
\def\taubf{\hbox{\boldmath$\tau$\unboldmath}}
\def\upsilonbf{\hbox{\boldmath$\upsilon$\unboldmath}}
\def\phibf{\hbox{\boldmath$\phi$\unboldmath}}
\def\chibf{\hbox{\boldmath$\chi$\unboldmath}}
\def\psibf{\hbox{\boldmath$\psi$\unboldmath}}
\def\omegabf{\hbox{\boldmath$\omega$\unboldmath}}
\def\Sigmabf{\hbox{$\bf \Sigma$}}
\def\Upsilonbf{\hbox{$\bf \Upsilon$}}
%\def\Phibf{\hbox{$\bf \Phi$}}
%\def\Psibf{\hbox{$\bf \Psi$}}
\def\Omegabf{\hbox{$\bf \Omega$}}
\def\Deltabf{\hbox{$\bf \Delta$}}
\def\Gammabf{\hbox{$\bf \Gamma$}}
\def\Thetabf{\hbox{$\bf \Theta$}}
\def\Lambdabf{\mbox{$ \bf \Lambda $}}
\def\Xibf{\hbox{\bf$\Xi$}}
\def\Pibf{{\bf \Pi}}
%\def\thetabf{\hbox{\boldmath$\theta$\unboldmath}}
\def\thetabf{{\mbox{\boldmath$\theta$\unboldmath}}}
%\def\thetabf{\hbox{$\bf{\theta}$}}
\def\Upsilonbf{\hbox{\boldmath$\Upsilon$\unboldmath}}
\newcommand{\Phibf}{\mbox{${\bf \Phi}$}}
\newcommand{\Psibf}{\mbox{${\bf \Psi}$}}
\def\olambda{\mathfrak{o}(\lambda)}
\def\complex{\mathfrak{C}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Calligraphic
\def\Ac{{\cal A}}
\def\Bc{{\cal B}}
\def\Cc{{\cal C}}
\def\Dc{{\cal D}}
\def\Ec{{\cal E}}
\def\Fc{{\cal F}}
\def\Gc{{\cal G}}
\def\Hc{{\cal H}}
\def\Ic{{\cal I}}
\def\Jc{{\cal J}}
\def\Kc{{\cal K}}
\def\Lc{{\cal L}}
\def\Mc{{\cal M}}
\def\Nc{{\cal N}}
\def\Oc{{\cal O}}
\def\Pc{{\cal P}}
\def\Qc{{\cal Q}}
\def\Rc{{\cal R}}
\def\Sc{{\cal S}}
\def\Tc{{\cal T}}
\def\Uc{{\cal U}}
\def\Vc{{\cal V}}
\def\Wc{{\cal W}}
\def\Xc{{\cal X}}
\def\Yc{{\cal Y}}
\def\Zc{{\cal Z}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%mathbb
\def\Abb{{\mathbb A}}
\def\BBb{{\mathbb B}}% different
\def\Cbb{{\mathbb C}}
\def\Dbb{{\mathbb D}}
\def\Ebb{{\mathbb E}}
\def\Fbb{{\mathbb F}}
\def\Gbb{{\mathbb G}}
\def\Hbb{{\mathbb H}}
\def\Ibb{{\mathbb I}}
\def\Jbb{{\mathbb J}}
\def\Kbb{{\mathbb K}}
\def\Lbb{{\mathbb L}}
\def\Mbb{{\mathbb M}}
\def\Nbb{{\mathbb N}}
\def\Obb{{\mathbb O}}
\def\Pbb{{\mathbb P}}
\def\Qbb{{\mathbb Q}}
\def\Rbb{{\mathbb R}}
\def\Sbb{{\mathbb S}}
\def\Tbb{{\mathbb T}}
\def\Ubb{{\mathbb U}}
\def\Vbb{{\mathbb V}}
\def\Wbb{{\mathbb W}}
\def\Xbb{{\mathbb X}}
\def\Ybb{{\mathbb Y}}
\def\Zbb{{\mathbb Z}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%command abbreviations
\newcommand{\bp}{\begin{psfrags}}
\newcommand{\ep}{\end{psfrags}}
\newcommand{\bl}{\begin{lemma}}
\newcommand{\el}{\end{lemma}}
\newcommand{\bt}{\begin{theorem}}
\newcommand{\et}{\end{theorem}}
\newcommand{\bc}{\begin{center}}
\newcommand{\ec}{\end{center}}
\newcommand{\bi}{\begin{itemize}}
\newcommand{\ei}{\end{itemize}}
\newcommand{\ben}{\begin{enumerate}}
\newcommand{\een}{\end{enumerate}}
%\newcommand{\bd}{\begin{definition}}
\newcommand{\ed}{\end{definition}}
\def\beq{\vskip .1cm \begin{equation}}
\def\eeq{\end{equation} \vskip .1cm \noindent}
\def\beqn{\vskip .1cm \begin{eqnarray}}
\def\eeqn{\end{eqnarray} \vskip .1cm \noindent}
\def\beqnn{\vskip .01cm \begin{eqnarray*}}
\def\eeqnn{\end{eqnarray*} \vskip .01cm \noindent}
\def\endproof{\hfill\blacksquare}
\def\defeq{:=}
\newcommand{\bim}{\begin{mylist}}
\newcommand{\eim}{\end{mylist}}
\def\bcase{\vskip .1cm \begin{numcases}}
\def\ecase{\end{numcases} \vskip .1cm \noindent}
\def\bsbcase{\vskip .1cm \begin{subnumcases}}
\def\esbcase{\end{subnumcases} \vskip .1cm \noindent}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%theorems

%\newtheorem{theorem}{Theorem}
%\newtheorem{corollary}{Corollary}
%\newtheorem{lemma}{Lemma}
%\newtheorem{definition}{Definition}
%\newtheorem{problem}{Problem}
%\newtheorem{assumption}{A}
%\newtheorem{properties}{Properties}
%\newtheorem{conjecture}{Conjecture}
%\newtheorem{criterion}{Criterion}
%\newtheorem{proposition}{Proposition}
%\newtheorem{remark}{Remark}
%\newtheorem{notation}{Notation}
%\newtheorem{derivation}{Derivation}
%\newtheorem{proof}{Proof}
\newtheorem{claim}{Claim}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\matplottc}[1]{               % single matlab plot twocolumn
        \unitlength .45truein
        \begin{center}
        \begin{picture}(5,4.6)(1.05,.45)
        \special{psfile=#1.ps hscale=50 vscale=50}
        \end{picture}
        \end{center}
}
\newcommand{\matplotfp}[1]{               % single matlab plot fullpage
        \unitlength .45truein
        \begin{center}
        \begin{picture}(14,16)(.8,-1)
        \special{psfile=#1.ps hscale=100 vscale=100}
        \end{picture}
        \end{center}
}
\newcommand{\matplothp}[1]{               % single matlab plot halfpage
        \unitlength .45truein
        \begin{center}  \begin{picture}(14,7.5)(-1,.55)
        \special{psfile=#1.ps hscale=80 vscale=80}
        \end{picture}
        \end{center}
}
\newcommand{\matplothptop}[1]{               % single matlab plot halfpage
        \unitlength .45truein                % when figure is top of page
        \begin{center}  \begin{picture}(14,6.3)(-1,1.15)
        \special{psfile=#1.ps hscale=80 vscale=80}
        \end{picture}
        \end{center}
}
\newcommand{\matplotcc}[4]{             % two axis('square') plots side by side
        \vspace{2.8in}
        \special{psfile=#1.ps voffset=-10 hoffset=-22 vscale=52 hscale=52}
        \special{psfile=/user/xu/isl/matlab/psfiles/#2.ps voffset=-10 hoffset=213 vscale=52 hscale=52}
        \hspace*{\fill}\hspace*{0.35in}#3\hspace*{\fill}\hspace*{\fill}\hspace*{
0.35in}#4\hspace*{\fill} }
\newcommand{\matplottwo}[4]{             % two axis('normal') plots side by side
        \vspace{2.62in}
        \special{psfile=#1.ps voffset=-10 hoffset=-27 vscale=52 hscale=52}
        \special{psfile=#2.ps voffset=-10 hoffset=218 vscale=52 hscale=52}
        \vspace*{0.18in}
        \hspace*{\fill}\hspace*{-.05in}#3\hspace*{\fill}\hspace*{\fill}\hspace*{
0.65in}#4\hspace*{\fill} } %%
%% This is for making fancy paragraphs
%%
\def\psfancypar#1#2{\begingroup\def\par{\endgraf\endgroup\lineskiplimit=0pt}
               \setbox2=\hbox{\large\sc #2}
%              \showthe\lht2\showthe\baselineskip
               \newdimen\tmpht \tmpht \ht2 \advance\tmpht by \baselineskip
%              \showthe\tmpht
% Changed 10/2/89 rhr - t-bol -> Times-Bold for dvi2ps to dvips conversion
%              \font\hhuge=t-bol at \tmpht
               \font\hhuge=Times-Bold at \tmpht
               \setbox1=\hbox{{\hhuge #1}}
%              \showthe\ht1
               \count7=\tmpht \count8=\ht1
%  note that all this BS is necessary since TeX only does integer
%  divides and rounds all results
               \divide\count8 by 1000 \divide\count7 by \count8
%               \showthe\count7
               \tmpht=.001\tmpht\multiply\tmpht by \count7
%               \showthe\tmpht
%              \font\hhuge=t-bol at \tmpht
               \font\hhuge=Times-Bold at \tmpht
               \setbox1=\hbox{{\hhuge #1}}
               \noindent
                \hangindent1.05\wd1
               \hangafter=-2 {\hskip-\hangindent
               \lower1\ht1\hbox{\raise1.0\ht2\copy1}%
                \kern-0\wd1}\copy2\lineskiplimit=-1000pt}


\newenvironment{ap}{
\renewcommand{\thesection}{\mbox{Appendix }\Alph{section}}
\renewcommand{\thesubsection}{\Alph{section}.\arabic{subsection
}}
\renewcommand{\theequation}{\mbox{\Alph{section}.}\arabic{equation}}
}{
\renewcommand{\thesection}{\arabic{section}}
\renewcommand{\thesubsection}{\thesection.\arabic{subsection}}
\renewcommand{\theequation}{\arabic{equation}}
}
%\setlength{\footnoterulewidth}{0.5pt}

%\setlength{\floatsep}{0.1cm}

%\setlength{\textfloatsep}{0.1cm}

%\setlength{\intextsep}{0.1cm}

%\setlength{\abovecaptionskip}{0.1cm}
%
%\setlength{\belowcaptionskip}{0.1cm}
%
%\setlength{\topsep}{0.1cm}
%
%\setlength{\partopsep}{0.1cm}
%
%\setlength{\itemsep}{0.1cm}
%
\setlength{\parindent}{0mm}
%
%\setlength{\dbltextfloatsep}{0.1cm}
%
%\setlength{\dblfloatsep}{0.1cm}
%
%\addtolength{\abovedisplayskip}{-1.5em}
%
%\addtolength{\belowdisplayskip}{-1.5em}
%
%\setlength{\arraycolsep}{0.1cm}

%\def\boxit#1{\vbox{\hrule\hbox{\vrule\kern3pt
%        \vbox{\kern3pt#1\kern3pt}\kern3pt\vrule}\hrule}}
%\def\dag{{\cal y}}
%\def\reals{ { {\rm  I \kern-0.15em R }  } }
%\def\complex{ {\,{{\rm C} \kern-0.50em \raise0.20ex {  |}}\, }}


%
%\newtheorem{theorem}{Theorem}[chapter]
%\newtheorem{conjecture}{Conjecture}[chapter]
%\newtheorem{lemma}{Lemma}[chapter]
%\newtheorem{definition}{Definition}[chapter]
%\newtheorem{corollary}{Corollary}[chapter]


%\newcounter{remarknr}[chapter]
%\newenvironment{remark}{\vskip\baselineskip
%\stepcounter{remarknr}\noindent{\bf
%Remark~\theremarknr.}}{\ \hfill $\Box$ \vskip\baselineskip}
%\newcounter{examplenr}[chapter]
%\newenvironment{example}[1]{\vskip\baselineskip
%\stepcounter{examplenr}\noindent{{\bf
%Example~\thechapter.\theexamplenr}\hskip .8em #1\\}}{\ \hfill $\Box$
%\vskip\baselineskip}




%\newcommand{\x}{\mbox{${\bf x}(t)$}}
%\newcommand{\s}{\mbox{${\bf s}(t)$}}
%\newcommand{\n}{\mbox{${\bf n}(t)$}}
%\newcommand{\jj}{\mbox{${\bf j}(t)$}}
%\newcommand{\R}{\mbox{$\hat {\bf R}_{N}$}}
%\newcommand{\Rhat}{\mbox{$\hat {\bf R}$}}
%\newcommand{\A}{\mbox{${\cal A}$}}
%\newcommand{\Ad}{\mbox{${\cal A}^d$}}
%\newcommand{\D}{\mbox{${\cal D}$}}
%\newcommand{\M}{\mbox{{\bf M}}}
%\newcommand{\Tr}{\mbox{Tr}}
%\newcommand{\pbox}{\hfill $\Box$}
%\newcommand{\blankline}{\vskip\baselineskip\noindent}
%\def\Rxx{\Rbf_{\ssstyle X\kern-.1em X}}
%\def\rxx{\hbox{$\Rxx$}}
%\def\ryy{\hbox{$\Rbf_{\ssstyle YY}$}}
%\def\rxy{\hbox{$\Rbf_{\ssstyle XY}$}}\def\ryx{\hbox{$\Rbf_{\ssstyle YX}$}}
%\def\rxyT{\hbox{$\Rbf_{\ssstyle XY}^*$}}\def\ryxT{\hbox{$\Rbf_{\ssstyle YX}^*$}}
%\def\Rss{\Rbf_{\ssstyle SS}}
%\def\rss{\mbox{$\Rss$}}
%\def\Rnn{\Rbf_{\ssstyle NN}}
%\def\rnn{\hbox{$\Rnn$}}
%\def\rxxinv{\hbox{$\Rbf^{-1}_{\ssstyle XX}$}}
%\def\Rssinv{\Rbf^{-1}_{\ssstyle SS}}
%\def\rssinv{\hbox{$\Rssinv$}}
%\def\rzzinv{\Rbf^{-1}_{\ssstyle ZZ}}\let\rzzi=\rzzinv
%\def\hatrxx{\widehat{\Rbf}_{\ssstyle XX}}
%\def\hatrzz{\widehat{\Rbf}_{\ssstyle ZZ}}
%\def\hatrss{\widehat{\Rbf}_{\ssstyle SS}}
%\def\phstar{{\phantom{*}}}
%\let\rzzhat=\hatrzz \let\rxxhat=\hatrxx \let\Rxxhat=\rxxhat
%\let\ssstyle=\scriptscriptstyle
%\let\rsshat=\hatrss


% I add the following!
%\def\eqorneq{=\!\!\!\! ? \,\,}
%\def\ltornlt{? \!\!\!\!\! <}
%\def\sN{{\ssstyle N}}
%\def\sM{{\ssstyle M}}
%\def\sF{{\ssstyle F}}
%\def\sT{{\ssstyle T}}
%\def\sH{{\ssstyle H}}
%\def\sK{{\ssstyle K}}
%\def\sL{{\ssstyle L}}
%\def\sQ{{\ssstyle Q}}
%\def\sV{{\ssstyle V}}
%\def\cross{\!  \times  \!}
%\def\alphat{\alpha^{(t)}}
%\def\alphab{\alpha^{(b)}}
%\def\betat{\beta^{(t)}}
%\def\betab{\beta^{(b)}}
%\def\ATbf{{\bf A_\sT}}
%\def\AHbf{{\bf A_\sH}}
%\def\sspan{\mbox{\it span}}



\def\Kout{\setbox1=\hbox{\Huge\bf K}\hbox to
1.05\wd1{\hspace{.05\wd1}\special{
"/Times-BoldItalic findfont 25 scalefont setfont
/prKzip
{0 0 moveto (K) show} def
/dozip
{gsave
  /xp 0 def
  .08 -.04 0
  {
   setgray
  prKzip
%  /xp xp dx add def xp -.7 translate %for
  -.7 .4 translate} for
  1 setgray prKzip
  0 0 moveto
  0 setgray
  .5 setlinewidth
  (K) true charpath  stroke
 grestore
} def
dozip}}}
\def\Sout{\setbox1=\hbox{\Huge\bf S}\hbox to 1.05\wd1{\hspace{.05\wd1}\special{"
/Times-BoldItalic findfont 25 scalefont setfont
/prSzip
{0 0 moveto (S) show} def
/dozip
{gsave
  /xp 0 def
  .08 -.04 0
  {
   setgray
  prSzip
%  /xp xp dx add def xp -.7 translate %for
  -.7 .4 translate} for
  1 setgray prSzip
  0 0 moveto
  0 setgray
  .5 setlinewidth
  (S) true charpath  stroke
 grestore
} def
dozip}}}

%\newcommand{\thhat}{\mbox{${\hat{\thetabf}}_N$}}
%\newcommand{\thbar}{\mbox{${\bar{\thetabf}}_N$}}
%\newcommand{\etahat}{\mbox{${\hat{\etabf}}$}}
%\newcommand{\etabf}{\mbox{${\bf\eta}$}}
%\newcommand{\e}{\mbox{${\bf e}_k$}}
%\newcommand{\ehat}{\mbox{$\hat{\bf e}_k$}}
%\newcommand{\EWE}{\mbox{${\bf E}_s^{}{\bf WE}_s^*$}}
%\newcommand{\DPD}{\mbox{$\Dbf^*\Pbf_{\bf A}^{\perp} \Dbf$}}
%\newcommand{\EWEhat}{\mbox{$\hat{\bf E}_s^{}{\bf W}\hat{\bf E}_s^*$}}
%\newcommand{\E}{\mbox{{\rm E}}}
%\newcommand{\Efs}{\mbox{${\bf E}_s^{}$}}
%\newcommand{\En}{\mbox{${\bf E}_n^{}$}}
%\newcommand{\Eshat}{\mbox{$\hat{\bf E}_s^{}$}}
%\newcommand{\Lshat}{\mbox{$\hat {\bf \Lambda}_s^{}$}}
%\newcommand{\Ls}{\mbox{$ {\bf \Lambda}_s^{}$}}
%\newcommand{\Ln}{\mbox{$ {\bf \Lambda}_n^{}$}}
%\newcommand{\Ltilde}{\mbox{$\widetilde {\bf \Lambda}$}}
%\newcommand{\Enhat}{\mbox{$\hat{\bf E}_n^{}$}}
%\newcommand{\Lnhat}{\mbox{$\hat {\bf \Lambda}_n^{}$}}
%\newcommand{\Ai}{\mbox{$ ({\bf A}^*{\bf A})^{-1} $}}
%\newcommand{\abf}{\mbox{${\bf a}$}}


%Define affiliation at footnote
% Make \small be smaller (8 pt)
%\def\small{\@setsize\small{9pt}\viiipt\@viiipt\let\@listi\@listI}


%%%%% notation %%%%%
%Anima added
\DeclareMathOperator{\Map}{Map}
\def\convp{{\stackrel{\mathrm{P}}{\to}}}

\def\qed{\hfill\hbox{${\vcenter{\vbox{
    \hrule height 0.4pt\hbox{\vrule width 0.4pt height 6pt
    \kern5pt\vrule width 0.4pt}\hrule height 0.4pt}}}$}}

\def\Depth{\delta}
\def\Hops{{\mbox{Hops}}}

% Variables
\newcommand{\wloc}{W} % graph
\newcommand{\loc}{L}
\newcommand{\wpre}{c}
%\newcommand{\neighbors}{\mathcal{N}}
%\newcommand{\clneighbors}{\mathcal{N}^{CL}}
%\newcommand{\nodes}{\mathcal{V} \cup \mathcal{H}}
%\newcommand{\onodes}{\mathcal{V}}
%\newcommand{\hnodes}{\mathcal{H}}
%\newcommand{\inodes}{\mathcal{I}}

\newcommand{\rc}{r}
\newcommand{\idtree}{\mathcal{T}_I}
\newcommand{\tree}{T}
\newcommand{\cltree}{\tree^{CL}}
\newcommand{\subtree}{\mathcal{S}}

% Vincent added
\newcommand{\calV}{\mathcal{V}}
\newcommand{\WW}{W}
\newcommand{\calE}{\mathcal{E}}
\newcommand{\calX}{\mathcal{X}}
\newcommand{\calA}{\mathcal{A}}
\newcommand{\calB}{\mathcal{B}}
\newcommand{\bX}{\mathbf{X}}
\newcommand{\bK}{\mathbf{K}}
\newcommand{\bx}{\mathbf{x}}
\newcommand{\bd}{\mathbf{d}}
\newcommand{\calH}{\mathcal{H}}
\newcommand{\hp}{\hat{p}}
\newcommand{\hd}{\hat{d}}
\newcommand{\hPhi}{\hat{\Phi}}
\newcommand{\hbd}{\hat{\bd}}
\newcommand{\hmu}{\hat{\mu}}
\newcommand{\calG}{\mathcal{G}}
\newcommand{\calC}{\mathcal{C}}
\newcommand{\calD}{\mathcal{D}}
\newcommand{\calT}{\mathcal{T}}
\newcommand{\bN}{\mathbb{N}}
\newcommand{\hT}{\hat{T}}
\newcommand{\ML}{\mathrm{ML}}
\newcommand{\Sg}{\mathrm{Sg}}
\newcommand{\calO}{\mathcal{O}}
%\newcommand{\Path}{\mathrm{Path}}
\newcommand{\diam}{\mathrm{diam}}
\newcommand{\MST}{\mathrm{MST}}
\newcommand{\Leaf}{\mathrm{Leaf}}
\newcommand{\brho}{\bm{\rho}}
\newcommand{\bSigma}{\bm{\Sigma}}
\newcommand{\bDelta}{\bm{\Delta}}
%\newcommand{\nbd}{\mathrm{nbd}}
\newcommand{\bR}{\mathbb{R}}

%\DeclareMathOperator*{\argmax}{argmax}
%\DeclareMathOperator*{\argmin}{argmin}

\newtheorem{THEO}{\bf Theorem}
\newtheorem{CORL}[THEO]{\bf Corollary}
\newtheorem{LEMM}[THEO]{\bf Lemma}
\newtheorem{REMA}{\bf Remark}
\newtheorem{DEFI}{\bf Definition}
\newtheorem{CLAIM}{\bf Claim}
\newtheorem{PROP}[THEO]{\bf Proposition}
\newtheorem{PROOF}{\bf Proof}
\newtheorem{EXAMPLE}{\bf Example}
\newtheorem{FACT}{\bf Fact}


\newcommand{\mathdef}{:=}
\DeclareMathOperator{\Tr}{Tr}
\DeclareMathOperator{\mat}{mat}
\DeclareMathOperator{\Rank}{Rank}

\def\nbd{\mathcal{N}}
\def\Path{{\mathrm{Path}}}

\DeclareMathOperator{\dist}{dist}
\DeclareMathOperator{\polylog}{polylog}
\def\veps{\varepsilon}
%\newcommand{\calX}{\mathcal{X}}
%\newcommand{\qed}{\hfill \ensuremath{\Box}}
%\newcommand{\bX}{\mathbf{X}}
\newcommand{\by}{\mathbf{y}}
\newcommand{\ba}{\mathbf{a}}
%\newcommand{\calG}{\mathcal{G}}
\newcommand{\calS}{\mathcal{S}}
\newcommand{\calN}{\mathcal{N}}
%\renewcommand{\calE}{E}
\newcommand{\hcalU}{\widehat{\mathcal{U}}}
%\renewcommand{\calV}{V}
%\newcommand{\calB}{\mathcal{B}}
%\newcommand{\calT}{\mathcal{T}}
%\newcommand{\calA}{\mathcal{A}}
%\newcommand{\calD}{\mathcal{D}}
%\newcommand{\bx}{\mathbf{x}}
%\newcommand{\0}{\mathbf{0}}
%\newcommand{\bR}{\mathbb{R}}
\newcommand{\calP}{\mathcal{P}}
\newcommand{\calY}{\mathcal{Y}}
%\newcommand{\calH}{\mathcal{H}}
\newcommand{\calU}{\mathcal{U}}
\newcommand{\bP}{\mathbb{P}}
\newcommand{\bE}{\mathbb{E}}
\newcommand{\bL}{\mathbf{L}}
%\newcommand{\bSigma}{\bm{\Sigma}}
\newcommand{\bmeta}{\bm{\eta}}
\newcommand{\bs}{\mathbf{s}}
\newcommand{\bxi}{\bm{\xi}}
%\newcommand{\bK}{\mathbf{K}}
\newcommand{\bzero}{\mathbf{0}}
\newcommand{\one}{\mathbf{1}}
%\newcommand{\hp}{\widehat{p}}
%\newcommand{\argmin}{\operatornamewithlimits{argmin}}
%\newcommand{\argmax}{\operatornamewithlimits{argmax}}
\newcommand{\hP}{\widehat{P}}
\newcommand{\hrho}{\widehat{\rho}}
\newcommand{\hPML}{{P}_{{\text{\tiny ML}}}}
\newcommand{\hI}{\widehat{I}}
\newcommand{\hQ}{\widehat{Q}}
\newcommand{\PML}{P_{\mathrm{ML}}}
\newcommand{\hTML}{{T}_{\text{\tiny ML}}}
%\newcommand{\Path}{\mathrm{Path}}
\newcommand{\tilp}{\widetilde{p}}
\newcommand{\tilJ}{\widetilde{J}}
\newcommand{\tilP}{\widetilde{P}}
\newcommand{\tilQ}{\widetilde{Q}}
\newcommand{\tilK}{\widetilde{K}}
\newcommand{\beps}{\bm{\epsilon}}
\newcommand{\var}{\mathrm{Var}}
%\newcommand{\etal}{et al.\ }
\newcommand{\hcalE}{{\calE}_{{\text{\tiny ML}}}}

\newcommand{\boxedeqn}[1]{%
  \[\fbox{%
      \addtolength{\linewidth}{-2\fboxsep}%
      \addtolength{\linewidth}{-2\fboxrule}%
      \begin{minipage}{\linewidth}%
      \begin{equation}#1\end{equation}%
      \end{minipage}%
    }\]%
}

\newtheorem*{theo}{Theorem}
\newtheorem*{proposition}{Proposition} 

\renewcommand{\thefootnote}{}





\newcommand{\fhcomment}{\textcolor[rgb]{1,0,0}{FH: }\textcolor[rgb]{1,0,0}} 
\renewcommand{\thefootnote}{}
\DeclareMathOperator{\Pairs}{Pairs}
\newcommand{\llvert}{\left\vert\vphantom{\frac{1}{1}}\right.}
\newcommand{\Pvalue}{\mathsf{P_{\text{val}}}}
\newcommand{\HRule}{\rule{\linewidth}{0.1mm}}
\def\nbd{\mathcal{N}}
\def\Path{{\mathrm{Path}}}

\def\veps{\varepsilon}
\newcommand{\Toep}{\mathsf{Cir}}
\DeclareMathOperator{\opt}{opt}
\newcommand{\DFT}{\mathsf{FFT}}
\newcommand*{\hermconj}{^{\mathsf{H}}}
\newcommand\supp{\operatorname{supp}}
\renewcommand{\thefootnote}{}
\def\veps{\varepsilon}
\DeclareMathOperator{\Cum}{C_3}
\DeclareMathOperator{\myblock}{blk}
\def\nbd{\mathcal{N}}
\def\Path{{\mathrm{Path}}}
\newcommand{\thetastar}{\ensuremath{\theta^*}}
\newcommand{\Astar}{\ensuremath{A^*}}
\newcommand{\Xstar}{\ensuremath{X^*}}
\newcommand{\iprod}[2]{\langle #1, #2 \rangle}
\newcommand{\Aiter}[1][t]{\ensuremath{A(#1)}}
\newcommand{\Aiteri}[1][t]{\ensuremath{A_i(#1)}}
\newcommand{\R}{\ensuremath{\mathbb{R}}}
\newcommand{\order}{\ensuremath{\mathcal{O}}}
\newcommand{\Xiter}[1][t]{\ensuremath{X(#1)}}
\newtheorem{assumption}{Assumption}
\newtheorem{goal}{Goal}
\newcommand{\Nb}{\text{nbd}}
\DeclareMathOperator{\Adj}{\mathcal{N}}
\def\ourframework{{$\textsf{ConvDic}$$+$$\textsf{DeconvDec}$ }}




==> include/talks/supp_packages.tex <==
\usepackage[mathscr]{eucal}
\usepackage{bm,verbatim,pifont,color,amssymb,amsfonts,amsmath,graphicx,epsf,psfrag,ifpdf,xmpmulti,cases,hyperref}
% \usepackage{slashbox}
\usepackage[english]{babel}
\usepackage[fleqn,tbtags]{mathtools}
\usepackage{amsmath}
\usepackage[attachfiles]{media9}
\usepackage{mathtools}
\usepackage{media9}
%\usepackage{multimedia}
\usepackage{pgfpages}
\usepackage{siunitx}
\usepackage{tablefootnote}
\usepackage{xspace}



\usepackage{tcolorbox}
%\usepackage{pgfpages}
%\usecolortheme{seagull}
%\definecolor{uofsgreen}{rgb}{.125,.5,.25}
%\usecolortheme[named=orange]{structure}
%\usecolortheme{rose}
%\usecolortheme{lily}
%\usecolortheme{rose}
%\usecolortheme{dolphin}
%\usecolortheme[rgb={0,0.17,0.45}]{structure}


%\usecolortheme{default}
%\usepackage[english]{babel}
% or whatever

%\usepackage[latin1]{inputenc}
% or whatever

\usepackage{colortbl}
%\usepackage{times}
%\usepackage[T1]{fontenc}
\usepackage{multimedia}
%\usepackage{latexsym, amssymb, amsmath}
%\setcounter{tocdepth}{3}
%\usepackage{graphicx}
%\usepackage{url}
%\usepackage{color}
%\usepackage{bm}
\usepackage{multirow}

%\usecolortheme{whale}
% \usecolortheme{beetle}
%\usecolortheme[named=seahorse]{structure}
%seahorse% seagull %beaver  albatross % lily %albatross %beetle %whale %crane
%\usecolortheme{default}
%\usepackage[english]{babel}
% or whatever
%
%\usepackage[latin1]{inputenc}
% or whatever
%
%\usepackage[lined, algonl, boxed]{algorithm2e}

\usepackage{algorithmic}
\usepackage{algorithm}
%\usepackage{subfigure}
%\usepackage{times}
%\usepackage[T1]{fontenc}
%\usepackage{hyperref}
%\usepackage{multimedia}
%\usepackage{latexsym, amssymb, amsmath}
%\setcounter{tocdepth}{3}
%\usepackage{graphicx}
%\usepackage{url}
%\usepackage{color}
%\usepackage{bm}
